DynoLoc: Infrastructure-free RF Tracking in Dynamic Indoor Environments

Promising solutions exist today that can accurately track mobile entities indoor using visual inertial odometry in favorable visual conditions, or by leveraging fine-grained ranging (RF, ultrasonic, IR, etc.) to reference anchors. However, they are unable to directly cater to "dynamic" indoor environments (e.g. first responder scenarios, multi-player AR/VR gaming in everyday spaces, etc.) that are devoid of such favorable conditions. Indeed, we show that the need for "infrastructure-free", and robustness to "node mobility" and "visual conditions" in such environments, motivates a robust RF-based approach along with the need to address a novel and challenging variant of its infrastructure-free (i.e. peer-to-peer) localization problem that is latency-bounded - accurate tracking of mobile entities imposes a latency budget that not only affects the solution computation but also the collection of peer-to-peer ranges themselves. In this work, we present the design and deployment of DynoLoc that addresses this latency-bounded infrastructure-free RF localization problem. To this end, DynoLoc unravels the fundamental tradeoff between latency and localization accuracy and incorporates design elements that judiciously leverage the available ranging resources to adaptively estimate the joint topology of nodes, coupled with robust algorithm that maximizes the localization accuracy even in the face of practical environmental artifacts (wireless connectivity and multipath, node mobility, etc.). This allows DynoLoc to track (every second) a network of few tens of mobile entities even at speeds of 1-2 m/s with median accuracies under 1-2 m (compared to 5m+ with baselines), without infrastructure support. We demonstrate DynoLoc's potential in a real-world firefighters' drill, as well as two other use cases of (i) multi-player AR/VR gaming, and (ii) active shooter tracking by first responders.

==> background/1-intro.tex <==
%challenge, motivation
%back + rel work = infra, imu ..dyn environment -> gap ..[ latency bound, infra free] -> challenges

RF based ranging is well studied in a lot of different application contexts spanning different wireless technologies. Some of the existing works promise extremely good ranging accuracies, often in the order of centimeters under ideal conditions. For instance, commercially available beacons using Ultra Wideband (UWB) technology already offers fine-grained ranging with an average accuracy of 10 centimeters. However, note that {\em ranging} does not automatically translate to {\em localization}. Localization involves calibrating the physical space with a set of known reference points or anchors. Ranges or distances of the given node needs to be estimated from four or more of such reference points in order to localize the node in the referenced 3D coordinate space using a technique typically referred as multilateration. 

\mypara{The Range vs. Localization Gap:} In this paper, we exclusively focus on the problem of infrastructure-free localization where direct multilateration is not applicable due to unavailability of known reference points or fixed anchors. Inertial sensors have long been used to track individual nodes however they show significant drift with time accumulating huge localization errors. Relative localization among the nodes is a feasible option in such scenarios. Several algorithms have been proposed to this end that essentially address the problem of relative localization in such sensor networks. This involves estimating the inter-nodal ranges across node pairs and using such distances to construct the relative geometry of the system of nodes. Much of the theoretical analysis done on this problem assumes an ideal deployment of nodes that does not hold in practice. For instance,~\cite{x,y,z} consider that ranges can be possibly estimated between any pair of nodes irrespective of their actual distance. This is not the case in reality when communication between nodes can be blocked by obstacles or just the sheer physical distance does not allow a communication link. Second, some of such studies~\cite{x, y, z} assume favorable, dense topologies such that every node has atleast a few neighbors to range. Third and most importantly, almost all of the works do not take into account how such ranges are collected across the nodes. All of such algorithms are snapshot based: once ranges are available it estimates the best fit for the relative geometry that minimizes range errors. However in reality collection of such ranges is a time consuming operation, and particularly in a dynamic unknown environment when nodes are mobile, the range collection needs to be as fast as possible. This poses a serious challenge when the system scales to few tens of nodes or the nodes have high mobility. It requires an intelligent way to select the right node pairs for ranging so as to create the relative geometry for the node locations with a minimal set of estimated ranges. Not only that, the range estimation accuracy needs to be taken into account as few of such ranges might be erroneous due to strong multipath issues or where direct LOS communication is blocked.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Inertial sensors (IMUs) have long been used to address the problem of indoor localization where dedicated infrastructure is absent or sparingly present. However IMUs, often low cost, just by itself cannot provide a high degree of localization accuracy even with state-of-the-art tracking algorithms~\cite{}. Hence many current approaches~\cite{} including commercial ones~\cite{} employ a hybrid solution that fuses an RF-based ranging modality to inertial sensor data. Many precise RF-based ranging modalities are available today including Ultra Wideband (UWB) or the Wi-Fi Fine Time Measurement (FTM). For instance, UWB can provide ranging precision in the order of 10 centimeters~\cite{} while Wi-Fi FTM provides a ranging accuracy of few meters ($\approx$\,5 meters)~\cite{}. Many solutions~\cite{} that adopt such ranging modalities make use of a few fixed nodes designated as \textit{anchors} which are assumed to be at known locations. The remaining nodes take turn in ranging with the anchor nodes and estimate their respective locations by multilateration. 

However this is often not a favorable setup for time critical missions, for instance, emergency response or public safety operations. Although it is true that in absence of anchors at known locations, it becomes a challenge to locate the nodes in an absolute sense, however even figuring out their relative positions poses a set of non-trivial challenges. Relative localization implies estimating a relative geometry for the set of nodes which in turn involves estimating \textit{pair-wise} ranges among them. Now, for a reasonable number of nodes (e.g., few tens) the number of such pair-wise ranges that need to be estimated can be very large (e.g., few hundreds to few thousands). A protocol that can infer such ranges will at least consume few tens of seconds to complete. Given the real-time requirements, a time lag of such scale will render the system unusable. In the following we layout the set of challenges associated with estimating the relative geometry for the nodes. Next, we discuss how the lack of infrastructure makes it even more challenging to align the relatively localized nodes with respect to a building map.

%we need an intelligent mechanism to orchestrate the ranging operation
%requires edges to be collected .. summarize challenges in nutshell .. glue missing that puts them together.
%also theoretical frameworks exists like mds sdr and so on. talk about relative localization 
%argue the critical aspects from a real-time system perspective. accuracy is important but at the same time latency or lag. 
%absolute location in a nutshell. relative localization can be discussed. the basis of localization technique depends on peer-to-peer range measurements. but needs to be gathered as fast as possible due to strict deadline requirements.
%however choosing the right set of nodes for ranging poses a complicated set of challenges.

\subsubsection{Challenge 1: Lack of Dedicated Anchors}
%
All nodes in our case are potentially mobile, thus lacking fixed locations. Therefore, there are no ``anchor" nodes or fixed nodes with known locations in our setting.
%
There are two implications of this - i) some of the time-efficient localization techniques such as Time Difference of Arrival (TDOA) \cite{tdoa} etc. cannot be used as it requires fixed anchors and wired connection between them for fine grained clock-synchronization. ii) localization depends on pairwise distance-measurement or ranges between nodes. In this case, without any  information about the topology resulting the wireless connectivity, the simplest approach would be to range a node with rest of the nodes, and then relatively localize the nodes using the geometry resulting from the set of pairwise ranges and repeat the operation to continuously localize each node. However, for $n$ nodes, it would require $^nC_2$ ranges.
Each ranging operation is time-consuming and cannot be arbitrarily minimized. For example, due to the broadcast nature of the wireless medium, each pair of nodes has to take turn in Time Division Multiple Access (TDMA) fashion for interference-free accurate ranging. Each ranging operation may take tens of milliseconds depending on the modality (WiFi, Ultra Wide Band etc.), data-rate of frame-exchange (110kbps,  64Mbps etc), frame-exchange protocols (single-sided and double-sided Two-way ranging \cite{twr} etc ), sampling rate and latency of the underlying electronics \cite{deca-chip-perf} and so on. For example, in our case, we are using double-sided two-way ranging protocol which requires 4 frame exchanges between each pair. We are using  UWB with a datarate of 110kbps, which requires a TDMA  slot time is 8msec for a maximum 110Bytes of payload. Therefore, each ranging takes 8$\times$4 = 32 msec. We are collecting all ranges using UDP frame via WiFi channel. The request and response alone takes about  2$\times$4=8msec. Therefore, each operation of range collection takes minimum 32+8 = 40msec. If there are 16 nodes, according to the above simplest method, we need to gather $^{16}C_2=120$ ranges to determine the geometry of relative localization. Therefore, the gap between successive localization of each node is at least 120$\times$40= 4800msec. However, if we had 3 static anchors covering the whole area of interest, each node could be localized in 3$\times$40=120msec after 3 ranging with 3 anchors, and for 16 nodes, collection of all possible ranges would take 16$\times$120 = 1920msec. The localization delay for the case without any dedicated anchors and with 3 anchors are \textit{quadratic} and \textit{linear} respectively in the \# of nodes. Therefore, the biggest challenge here is to minimize the localization delay by scheduling only a subset of all possible  $^nC_2$ ranges, taking into consideration factors such as link or range quality, node mobility, effect on the relative geometry etc. Therefore, the lack of dedicated anchors requires complex orchestration of ranging operations among nodes, to scale localization with the \# of nodes and to minimize the delay.
\end{comment}
%

==> background/3-relative-localization.tex <==
\subsection{Geometric Rigidity}
\begin{figure}[!tbh]
	\centering
	\includegraphics[width = 0.95\linewidth ]{figs/trans-rot-flip.png}
	\caption{Translation, Rotation and Flip}
	\label{fig:node-trans-rot-flip}
\end{figure}
\vspace{0.1in}
As discussed before, nodes can be relatively localized with respect to each other using pairwise ranges.
%
These ranges (edges) along with nodes (vertices) form a graph representing the relative geometry.
%
By rotating, translating and flipping the local coordinate of this graph\footnote{using additional information from IMU, floor-plan etc.}, we can derive the absolute locations of all the nodes as shown in Figure \ref{fig:rel-graph}. Therefore, in our problem, localization involves relative localization followed by absolute localization.
%
%real time, time constraint
However, the nodes can be mobile. Therefore, localization is done in real time and continuously.
%
If all possible ranges are collected in orderly fashion, the approach is deterministic and the resulting relative geometry (a clique) is unambiguous (See Figure \ref{fig:rigidity}(a)).  
%
However, there are two issues: 
%

\noindent i) \textit{Connectivity constraint}: Due to limited ranging capability, ranges for all pairs of nodes are not always available. 
%

\noindent ii) \textit{Time constraint}: Collection of ranges for all pairs of nodes may require  prohibitively high amount of time as discussed before.
%For example, for 20 nodes and ranging time of 8 msec, it would take $^{20}C_2\times{}8=1520$ msec. For a given time budget, say 1sec, we can collect 65\% of the all possible ranges.
%

As a result of the above two constraints, only a subset of edges are available to form the relative geometry. However, a random subset of the edges won't guarantee unambiguous graph. To this end, we introduce the notion of graph ``rigidity". As shown in Figure \ref{fig:rigidity}, equal \# of edges are taken to form two subgraphs as in (b) and (c) from the complete graph in (a). The graph in (b) is not rigid, as node 1 can freely move around. But graph in (c) is rigid discounting the effect of translation, rotation and flip. If the resulting graph is not rigid, relative localization will fail. Therefore, it requires careful selection of edges in a given time budget. For example, the graph in (a) and (c) are both rigid and will result in the same relative localization. Yet, (a) uses 28 edges and (c) uses 16. Therefore, the orchestration to collect only sufficient number of ranges to relatively localize the nodes, is challenging.

\begin{comment}
%Geometry
\subsubsection{Challenge 4: Geometric Requirements}.
%concept of relative and absolute location
Without at least three (in 2D) fixed anchors with known location, we need to first derive the relative locations of the nodes from the pairwise ranges. To this end, we derive relative locations by forming  a ``rigid graph" with all the nodes on it. This graph can be translated and/or rotated to derive the absolute location of each node. The requirements of this rigid graph formation put additional constraints on the ranging operation as described below.
To elucidate the inherent  geometric challenges of relative localization, let us first introduce some relevant terms from computational geometry.\footnote{Unless otherwise stated, the scenario is for 2D space, although it can be generalized for 3D.}

\uterm{Distance Geometry Problem (DGP)} A \textit{realization} is a function that maps a given set of vertices to 2D Euclidean space. Given a simple, connected, weighted graph $G=(V, E, d)$, where $V$ is the set of vertices, $E$ is the set of edges and $d(u, v)$ is the Euclidean distance or range between nodes $u, v \in V$,  the DGP problem is to find whether there is a realization $x:V \rightarrow{} \mathbb{R}^2$ such that each range is preserved i.e $\forall (u,v) \in E, \; ||x(u) - x(v)|| = d(u, v)$ where $||.||$ is the Euclidean norm.

As shown in \textcolor{red}{Figure \ref{fig:dgp-explanationi}}, given a set of inter-node distances, we can construct a quadrilateral of a specific shape which can be translated, rotated, or flipped resulting in infinite number of realizations with the same Euclidean congruence. However, in relative localization, only the shape matters. Therefore, in our case, the DGP problem is to find  whether there is any realization, or unique or countable or infinite number of realization discounting above three effects. Based on this notion, we can define rigidity as follows:

\uterm{Rigid Graph Formation Problem (RGFP)} A simple, connected, weighted graph $G=(V, E, d)$ is ``rigid" if there is only one realization discounting translation, rotation and flip. As shown in \textcolor{red}{Figure \ref{fig:rigid-graph}}, case (a) is rigid, it has only one realization, case (b) is not rigid, it has two realizations, case (c) is not rigid either, it has infinitely many realizations. In our case, determining graph rigidity has two benefits:
%
\begin{enumerate}[noitemsep, topsep = 0em]
    %
    \item Identify nodes that require additional information besides ranges for relative localization
    %
    \item Besides initial and periodic ranging on all available edges (formed due to wireless connectivity of the ranging modality), schedule ranging on a subset of the edges to  ensure maximum benefit (relative localization) with minimum cost (\# of edges). 
 \end{enumerate}   
 %
Note that, DGP is NP-hard (see Saxe's proof \cite{dgp-proof}) for any dimensional Euclidean space. As such, determining rigidity of arbitrary graph is also NP-hard. However, using graph property, we can formulate efficient signatures for rigidity as described in Section \ref{sec:method}. In our case, each edge represents a time-consuming ranging operation. Therefore, to minimize localization time, it is imperative  to find a maximal (highest number of vertices) rigid sub-graph, if any, using minimum number of edges. We can define the problem as follows.

\uterm{Minimally Rigid Maximal Sub-graph (MRMS) Problem (MRMSP)} Find a (vertex induced) rigid subgraph $G_r = (V_r, E_r)$ of a given simple, connected, weighted graph $G=(V, E, d)$, such that i) adding any new vertex $v \in (V-V_r)$ (along with the incident edges) to the sub-graph will make the sub-graph non-rigid and ii) removing a single edge from $E_r$ will render the sub-graph non-rigid. 

As shown in \textcolor{red}{Figure \ref{minimally-rigid}}, the input graph has 8 nodes, however it has a  sub-graph (5-clique) that is rigid. In the first step (see (b)), we can prune the nodes that cannot  be part of any rigid sub-graph. In the next step (see (c)), we can prune some edges making it minimally rigid. The resulting graph in (c) is MRMS. In our ranging operations, the MRMS edges are of utmost priority to form the rigid graph and hence compute the relative localization. We can add additional edges to MRMS, if the time budget permits, to meet the requirements of the other challenges discussed so far. Regardless, if the MRMS requirement is not carefully followed in the ranging operation, the relative localization will fail. For example in Figure \ref{fig:minimally-rigid}(d), the same number of edges as in (c) has been selected for ranging without considering their utility for MRMS formation, but the resulting sub-graph, although has all the vertices, still fails to be rigid. Therefore, ranging on the sequence of edges in (c) is always preferred to on those in (d) even though both sequences have equal \# of edges and hence require equal time. MRMS problem is NP-hard due to NP-hardness of DGP and Rigidity problem.

\uterm{Euclidean Distance Matrix (EDM) Completion and De-noising Problem (EDMCDP)} If all pairwise ranges ($^nC_2$ for $n$ nodes) are available, we can represent the edge-weight function $d$ as an n$\times{}$n matrix $D$, which is known as EDM. We can derive a $n$-node clique (which is a rigid graph \cite{edm}) from this EDM in polynomial time using standard algorithm \cite{cmds}.
However, in our case i) all pairwise ranges are not always available due to limited ranging capability (i.e. as low as 10m for NLOS UWB in our case) and sprawling indoor area (i.e 50m $\times{}$50m in our case).
 ii) the derived ranges (i.e. EDM entries) can be extremely noisy to the point of violating simple triangular inequality as illustrated in the previous challenge. Unfortunately, standard algorithm cannot be used for this EDM with incomplete and noisy entries.
  Therefore, the EDMCDP is to de-noise the ranges and complete the EDM before using standard algorithm to form the rigid graph.

\uterm{Absolute Localization Problem (ALP)} Once the rigid graph is formed, the next challenge is to derive absolute localization by translation and rotation operation\footnote{We mitigate the flip or reflection by following a specific vertex ordering and origin assignment, resulting from node ID's as discussed in Section \ref{sec:method}}. Determining the required translation $x_t$ and rotation $\theta$ from additional information such as IMU-heading, historical data of track of each node, floor-map etc. as shown in \textcolor{red}{Figure \ref{absolute-loc}} is also challenging.
%
\begin{figure}
\centering
\includegraphics[width = 0.65\linewidth ]{figs/geom-problem.png}
\caption{Hierarchy of Geometric Challenges}
\label{fig:geom-problem-hiearchy}
\end{figure}
\vspace{0.1in}
%
We can summarize the geometric challenges in our setting as shown in Figure  \ref{fig:geom-problem-hiearchy}.
\end{comment}

==> background/4-node-mobility.tex <==
%mobility
\subsection{Node Mobility}

A primary challenge in maintaining the relative geometry of the nodes as updated as possible stems from the mobility pattern of such nodes. The relative motion among the nodes determine the rate at which the inter-nodal distance varies. Let's call such inter-nodal distance an \textit{edge}. We demonstrate a scenario where multiple nodes move at uniform speeds on a building floor. Figure XX(a) shows the evolution of such edges with time. Note that every edge evolves at a different rate depending on the respective nodes' individual speed as well as the direction of their motion. 

\begin{figure}[!tbh]
	\centering
	\includegraphics[height=1.4in, width = 0.45\linewidth ]{figs/challenge_mobility_1.jpg}
		\includegraphics[height=1.4in, width = 0.45\linewidth ]{figs/challenge_mobility_2.jpg}
	\caption{Impact of node mobility on ranging uncertainty}
	\label{fig:node-mobility}
\end{figure}
\vspace{0.1in}

This poses a severe challenge in orchestrating the range measurements. As shown in figure XX(b), the frequency of such ranging measurements itself might bring different utilities when looking at individual edge uncertainties. The edges with a high degree of change need to scheduled more often compared to edges that have a limited change within a certain period of time. Also note that the total number of ranging measurements that can be scheduled within a given time is finite. Hence bundling the \textit{most updated} set of edges while performing the measurements is crucial.

==> background/5-channel.tex <==
%channel
\subsection{Channel Characteristics}
Due to node mobility, the link characteristics of each pair of nodes may change drastically. This adversely affects the ranging accuracy over time. When both nodes of a link are static, they are close by and they have line of sight (LOS) between them, we have the best scenario wherein, the channel characteristics remains unchanged, the received signal is strong and the effect of multi-path is minimal \cite{wireless-prop}. Hence, the ranging accuracy is high. However, we can have the following scenarios:
\begin{enumerate}[noitemsep, topsep = 0em]
    \item The inter-node distance can be high
    \item There is no line of sight (NLOS)
    \item one or both nodes are moving
\end{enumerate}
Any or a combination of the above scenarios affect ranging accuracy. In particular, for our case of time of flight-based ranging using UWB, with LOS, the maximum range turns out to be around 50 meter. However, in presence of obstacles such as walls, furniture etc, this range decreases drastically form 50 to 20 meters or so. In other words, the range is related to the number of obstacles in between the ranging nodes. When the nodes are moving in case of NLOS, we have the worst scenario and the ranging accuracy are the poorest. 
\\
%
\begin{figure}
\centering
\includegraphics[height=2.8in, width = 0.7\linewidth ]{figs/labeled-floor-map.png}
\caption{Indoor map with a pair of nodes in different settings}
\label{fig:indoor-map}
\end{figure}
\vspace{0.1in}
%
%
\begin{figure*}
\centering
\fbox{\includegraphics[width=0.95\textwidth, ]{figs/dummy/dummy-back.png}}
\caption{Ranging accuracy for diverse indoor  scenarios} 
\label{fig:indoor-cdf}
\end{figure*}
\vspace{0.1in}
%
To substantiate our claim, we create diverse scenarios with two nodes in an indoor environment as shown in Figure \ref{fig:indoor-map}. We then generate the CDF of ranging errors for all cases as shown in Figure  \ref{fig:indoor-cdf}. First, we keep both the nodes static in LOS and change the distance from 1 meter up to 40 meters. We observe that the resulting ranging error and its variance is very small and always under 0.25 meters. Now, we put the two nodes in NLOS locations again varying the distance from 1 meter up to 40 meters and also with varying number of walls (wall-count = 1, 2, 3 up to 12) between them. As shown in the figure, NLOS has worse accuracy than LOS but it only worsens with the increase of the number of walls. Finally, we move the nodes linearly with a relative speed between them from 0.5 and 2 m/sec for all the above scenarios. This time, the accuracy gets worse compared to the corresponding static scenarios. Out of all the cases, the scenario with the highest node mobility, NLOS with maximum wall/obstacle count has the poorest range and the worst accuracy of up to 10 meter.

We now show that, one or more low-accuracy ranges drastically reduces the localization accuracy. It requires at least three edges in the relative geometry  to localize a node. The core  of the solution for the localization without dedicated anchors is  the selection of edges for ranging. To illustrate the impact of edge-selection, we create a scenario with  7 static nodes as shown in  \textcolor{red}{Figure \cite{fig:edge-loc-quality}}. We want to localize node 1 which is incident with 6 edges marked as $e_{1k}$ for $k=1,\ldots,6$. We first collect the range values for all the six edges for long enough time. Then using ground truth of the pairwise distances between node 1 and the rest of the nodes,  we rank the edges in terms of the median ranging error as follows: $e_{11} < e_{12} < e_{13} < e_{14} < e_{15} < e_{16}$ ($e_{11}$ has the least ranging error). Also note that the 3 best accurate edges are LOS links, the rest are NLOS links and 2 of the LOS edges have a length more than those of NLOS edges. Therefore, unless LOS link, short range does not necessarily imply high ranging accuracy.
Let us consider the  scenarios of edge-selection and the resulting localization error using multilateral as shown in Table \ref{tab:accuracy}.
%
\begin{table}[h!]
\centering
 \begin{tabular}{||p{0.73in} | p{0.8in} | p{1.3in}||} 
 \hline \hline
 \textbf{Selected Edges} & \textbf{Localization Accuracy} & \textbf{Comment}\\ \hline
 $e_{11}$, $e_{12}$, $e_{13}$ & 20 cm & Best edges ensure least error  \\ \hline
  $e_{14}$, $e_{15}$, $e_{16}$ & 200 cm & Worst edges result in the worst error\\ \hline
  $e_{11}$, $e_{12}$, $e_{13}$, $e_{14}$, $e_{15}$, $e_{16}$ & 210 cm & No guarantee of accuracy despite all edges \\ \hline
    $e_{11}$, $e_{12}$, $e_{13}$, $e_{16}$ & 175 cm &  A Single ``bad" edge ($e_{16}$) affects accuracy\\ \hline \hline
 \end{tabular}
 \caption{Localization accuracy involving diverse edges}
\label{tab:accuracy}
\end{table}
%
The observation is as follows- multilateration does not take into account the accuracy of the edges. So, using more edges in it, does not guarantee improvement of localization accuracy. Rather, we need to rank the edges according to their ranging accuracy and only select the best ones for multilateration. Ranging on all incident edges, including the low-accuracy ones rather deteriorate the localization accuracy. However, these edge-rankings are not permanent, rather changing due to node mobility. Therefore, computing edge-ranks in the presence of arbitrary node mobility  and selecting a subset of them for localization to increase accuracy is indeed a challenging task. We use Channel Impulse Response (CIR) of the link to quantify its quality as discussed in Section \ref{sec:method}.

==> background/6-absolute-loc.tex <==
\subsection{Absolute Localization}
%
Once the relative geometry is determined, the next step is to absolutely localize all the nodes by determining the translation and rotation required to affix the rigid graph as a whole. For this purpose, at least one node with known location (beacon node) is required from which the distance and direction of the rigid graph is determined. To determine the direction or orientation of the rigid graph, the IMU, which gives the heading of the nodes relative to earth's north-south axis, is useful. Note that, without anchor nodes, dead-reckoning by IMU is a natural choice for localization via tracking, as it does not require any external set-up at all. However, displacement computed by IMU using the state-of-the-art methods \cite{IMU-survey}, can only be reliably used for few seconds due to run-away error as shown in Figure \ref{fig:imu-exp}. On the other hand, orientation or heading computed by the IMU is reliable over time as shown in Figure \ref{fig:imu-exp}. Additionally, indoor floor-map may be available, which further restricts the translation and rotation of the rigid graph. In summery, deriving absolute locations from relative ones fusing diverse set of information such as from IMU, floor-pan, path-history of the nodes etc. is very challenging in a dynamic environment and requires thoughtful design of systme and  methods. 
%
\begin{comment}
All nodes in our case are potentially mobile, thus lacking fixed locations. Therefore, there are no ``anchor" nodes or fixed nodes with known locations in our setting.
%
There are two implications of this - i) some of the time-efficient localization techniques such as Time Difference of Arrival (TDOA) \cite{tdoa} etc. cannot be used as it requires fixed anchors and wired connection between them for fine grained clock-synchronization. ii) localization depends on pairwise distance-measurement or ranges between nodes. In this case, without any  information about the topology resulting the wireless connectivity, the simplest approach would be to range a node with rest of the nodes, and then relatively localize the nodes using the geometry resulting from the set of pairwise ranges and repeat the operation to continuously localize each node. However, for $n$ nodes, it would require $^nC_2$ ranges.
Each ranging operation is time-consuming and cannot be arbitrarily minimized. For example, due to the broadcast nature of the wireless medium, each pair of nodes has to take turn in Time Division Multiple Access (TDMA) fashion for interference-free accurate ranging. Each ranging operation may take tens of milliseconds depending on the modality (WiFi, Ultra Wide Band etc.), data-rate of frame-exchange (110kbps,  64Mbps etc), frame-exchange protocols (single-sided and double-sided Two-way ranging \cite{twr} etc ), sampling rate and latency of the underlying electronics \cite{deca-chip-perf} and so on. For example, in our case, we are using double-sided two-way ranging protocol which requires 4 frame exchanges between each pair. We are using  UWB with a datarate of 110kbps, which requires a TDMA  slot time is 8msec for a maximum 110Bytes of payload. Therefore, each ranging takes 8$\times$4 = 32 msec. We are collecting all ranges using UDP frame via WiFi channel. The request and response alone takes about  2$\times$4=8msec. Therefore, each operation of range collection takes minimum 32+8 = 40msec. If there are 16 nodes, according to the above simplest method, we need to gather $^{16}C_2=120$ ranges to determine the geometry of relative localization. Therefore, the gap between successive localization of each node is at least 120$\times$40= 4800msec. However, if we had 3 static anchors covering the whole area of interest, each node could be localized in 3$\times$40=120msec after 3 ranging with 3 anchors, and for 16 nodes, collection of all possible ranges would take 16$\times$120 = 1920msec. The localization delay for the case without any dedicated anchors and with 3 anchors are \textit{quadratic} and \textit{linear} respectively in the \# of nodes. Therefore, the biggest challenge here is to minimize the localization delay by scheduling only a subset of all possible  $^nC_2$ ranges, taking into consideration factors such as link or range quality, node mobility, effect on the relative geometry etc. Therefore, the lack of dedicated anchors requires complex orchestration of ranging operations among nodes, to scale localization with the \# of nodes and to minimize the delay.
\end{comment}
%

==> background/junk.tex <==
\begin{comment}
%
In this section, we introduce terms and definitions related to our problem, illustrate the gap between accurate localization and accurate ranging and then, formally define the problem.
%
\uterm{Problem Statement} Given a set of potentially mobile nodes, each with a limited ranging capability, find the current location of each node using available pair-wise ranges, but without any anchor nodes, such that localization error is minimized.
 %
\begin{figure}
\centering
\includegraphics[ height=1.5in ]{figs/motion.png}
\fbox{\includegraphics[ height=1in ]{figs/blank}}
\caption{(a) Location Uncertainty (b) heatmap of localion uncertainty w.r.t. \# of nodes and \% of mobile nodes}
\label{fig:motion}
\end{figure}
\vspace{0.1in}
 %
Let there be $N$ nodes (either static or mobile) labeled $i \in \{1, 2, \ldots, N$\}. At any instant $t$, we denote the location of node $i$ by a $d$-dimensional vector $\mathbf{x}_i(t)$. Unless otherwise stated, we assume 2D localization i.e $d=2$. If all nodes are static, $\mathbf{x}_i(t)$ is computed once and remains the same for the rest of the time. However, node $i$ can be static or mobile spontaneously and in absence of any predefined mobility pattern\footnote{as in the case of visual-SLAM \cite{visual-slam}, indoor mapping \cite{indoor-mapping} etc}, the location $\mathbf{x}_i(t)$ has to be computed repeatedly for each node $i$. The difference between the true location $\mathbf{x}_i(t)$ and computed location $\mathbf{\hat{x}}_i(t)$ is the localization error $e_i(t)$. We want to minimize this error for all nodes and all instants. To capture the notion of this error, we assume that the maximum linear velocity of any node is $v_{max}$. This assumption is not impractical since, in our case, these nodes  represent human beings or robotic entities such as drones. In indoor areas, drones and other vehicles to be localized, have limited speed \cite{}. Studies such as \cite{firefighter-speed-study} also present maximum speed of emergency workers in indoor areas.
If the location of a node $i$ is computed at instant $t_1$ and then at instant $t_2$, the delay between successive localization is $\Delta t = t_2 - t_1$, and the  maximum possible  displacement of node $i$ from its earlier location $\mathbf{x}_i(t_1)$ is $\Delta t \times{} v_{max}$. We associate a circle of radius $\Delta t \times{} v_{max}$ centered at location $\mathbf{x}_i(t_1)$ representing the uncertainty of location of node $i$ for the duration between $t_2$ and $t_1$.
We want to limit this uncertainty for all nodes between successive localization. This uncertainty is representative of the instant localization error $e_i(t)$.
To minimize this error, it is desirable to  schedule the localization for all nodes repeatedly such that ``apparently static" nodes are localized less frequently (high $\Delta t$) than ``apparently dynamic" nodes (low $\Delta t$). 
%
In other words, we want to increase the localization-rate for all mobile nodes as best as possible under the existing system.
As presented in Section \ref{sec:applications}, this high localization-rate enables and props up applications such as visual tracking and fine-grained sensing. In these applications, both accurate and fast localization are of importance.
%
However, this requires complex orchestration of existing ranging techniques.
In this work, we tackle this challenge via multiple steps laid out in Section \ref{sec:method}. 

To make the case for the required orchestration of localization, we note that the localization of each node is not instant, rather takes some time $\Delta t_l$. Typically, some $k$ ``anchor" nodes with known locations are deployed in the area of interest. Each of the $N$ nodes with unknown location, determines their distance or range, from each of the $k$ anchors via different wireless modalities such as WiFi, Ultra Wide Band (UWB), Bluetooth etc, and via different techniques such as Time of Flight (TOF), Time Difference of Arrival (TDOA), Angle of Arrival (AOA) etc\footnote{A very rich literature already exists for accurate range calculation for different modalities and techniques. Therefore, accurate ranging is not the focus of this work. We only assume that no fixed set of anchor nodes are available.}. Given at least 3(4) such ranges from the anchors, each node can be localized in 2D (3D) using multi-lateration \cite{} technique. Regardless, of the modalities and techniques used, each ranging takes some time $\Delta t_r$. If $k$ such ranges are used in $k$-lateration, the localization time $\Delta t_l$ is at least $k\Delta t_r$, which can vary from few milliseconds to few seconds or even more, depending on ranging modality, technique, number of nodes, data-gathering protocol etc. We justified our choices of ranging modalities, techniques, protocols in Section \ref{subsec:our-choices}, and calculated the minimum value for ranging delay $\Delta t_r$ to be 40 milliseconds for our prototype. This value is the characteristic of the localization system and as such, puts a limit on the ranging rate. For example, in our prototype, the ranging rate is 1/(40 msec) = 25Hz. For trilateration, the localization rate is 25/3 $\approx$ 8Hz. For the case where 20 nodes are localized in rounds, the localization rate for individual node is 8/20 =  0.4Hz.  This location update rate may not be satisfactory for highly mobile nodes in many applications such as those in Section \ref{sec:applications}. Let us assume that $v_{max}=1ms^{-1}$. Therefore, the uncertainty $\Delta t \times v_{max}$ is 1/0.4 = 2.5meter despite ranging accuracy of one-tenth of a meter. This uncertainty only increases with the number of nodes. Lack of anchors, as in our case, makes the problem more complicated. However, there is a significant scope of improvement of both accuracy and localization-rate given a maximum ranging-rate in such a challenging setting. Therefore, the gap between  ``accurate ranging" and ``fast and accurate localization" still remains to be bridged. In this regard, we identify two challenges as follows.
\\ \noindent 1)\textit{ Challenges due to node-mobility}: Due to heterogeneous node mobility, highly mobile nodes suffer more instant localization error in case of uniform localization-rate. On the other hand, node mobility in our case is spontaneous and therefore, any static node can become mobile at any instant. As such, coordinating and scheduling a non-uniform localization for all nodes is itself challenging. 
\\ \noindent 2)\textit{ Challenges due to lack of anchors}: In case of $k$ anchors and $k$-lateration, the localization operation of each node is predictable and takes constant time. Also, anchors are carefully deployed for full coverage. However, lack of anchors make the problem immensely challenging. On one hand, no nodes have known absolute locations. However, it is possible to relatively localize the nodes with respect to each other. On the other hand, no nodes have fixed set of nodes to range with due to mobility. Some nodes may be out of ranges of every other nodes for a period of time. Such variability makes the localization operation unpredictable and impact both accuracy and speed of localization. Additionally, lack of anchors make some of the fastest and highly scalable localization technique such as TDOA with synchronized anchors \cite{} impractical. As such, the underlying technique requires Time Division Multiple Access (TDMA) of the wireless medium for ranging. TDMA ranging deteriorates localization rate with the increasing number of nodes. Finally, transforming relative locations to absolute ones using additional information such as floor-map, Inertial Measurement Unit (IMU) heading etc. on-the-fly requires concrete algorithm.
\end{comment}



==> ieeetran-final_sub/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method/1-intro.tex <==
\subsection{Background of Solution}
%
In absence of fixed anchor nodes, we localize all the nodes in two step i) \textit{relative localization}: we construct an unambiguous geometric shape called ``rigid graph" by measuring distances (called ranges) between the nodes ii) \textit{absolute localization}: using additional information such as heading from IMU etc., we rotate, translate or flip the rigid graph to derive absolute locations of the nodes with respect to a global coordinate.

In the relative localization step, based on the range measurements,  we generate an $n\times{}n$ matrix called Euclidean Distance Matrix (EDM)  for $n$ nodes. In EDM, the entry in the $i$-th row and $j$-th column is the range between node $i$  and $j$ (nodes are labeled 1 through $n$). Given all the pairwise ranges between the nodes i.e the EDM, we can form an unambiguous geometric shape called the rigid graph \cite{edm-graph} discounting rotation, translation and flip. However, each ranging operation takes tens of milliseconds which cannot be arbitrary reduced (out of scope of this work) for a given system. Given a fixed ranging time (say 40 msec), forming the EDM for even a small number of nodes (say 16) requires high number of measurements ($^{16}C_2 = 120$) and thus significant amount of time ($120\times{}40/1000=4.8$ sec). On the other hand, nodes are potentially mobile causing temporal inconsistency during formation of the EDM. Consider a range  measured first during the computation ($(120-1)*40/1000 = 4.76$ secs prior to the EDM completion). Due to the mobility of this node (say 1$ms^{-1}$), the first range will be way off the true value (at most $(1ms^{-1}\times{}4.76$ sec)$= 4.76$ meter). As such, the location of the node will also be  off (by at least few meters) the true location. Therefore, although a complete EDM guarantees an unambiguous rigid graph, it does not minimize localization error. Now consider the case, where we take subset of all possible ranges (say 32 ranges out of 120). Here, all the ranges will be fresher and more accurate (first measured range will be off by at most $(31\times{}40/1000)=1.24$ meter) than the  previous case. However, taking an arbitrary subset of ranges will not guarantee rigid graph (32 ranges will never form a rigid graph for 16 nodes). Also ranging between a pair of nodes will not be possible if they are out of each others wireless range. 

We want to find a ``sweet spot" between these two following cases - i) a full EDM rendering erroneous relative locations due to  temporal inconsistency and ii) incomplete EDM rendering no rigid graph despite fresher set of ranges. Therefore, the relative localization step entails  ``edge selection" step wherein, we select a subset of all possible edges for  ranging such that i) the rigid graph formation is guaranteed and ii) the localization error (due to the temporal inconsistency) is minimized. In other words, we want to form the rigid graph using minimum number of ranges. However, the underlying problem is NP-hard \cite{maximal-core}. Even for a small number of nodes ($16$), the number of choices is combinatorially explosive 
($2^{^{16}C_2}$, trillions of trillions of choices). Only a very tiny fraction of these choices actually result in a rigid graph (out of 1 million random choices, only XX\% resulted in rigid graph for $n=16$, this ratio decreases drastically with the increase in the number of nodes, see Figure \ref{fig:comb-edge-selection}). On top of that, only a tiny fraction (see Figure \ref{fig:comb-edge-selection}) of these choices rendering a rigid graph actually result in high-accuracy localization. This indeed is the proverbial ``needle in the haystack" search.
However, we do not have endless time to compute a single snapshot of locations, due to constant mobility of the nodes. Therefore, finding the desired sweet spot between a fully complete and an almost incomplete EDM is indeed very challenging yet rewarding task for high-accuracy localization. 
%

Once we derive an incomplete EDM, the next task is to fill in the missing values. There are many algorithms \cite{edm-completion} for this purpose. However, two incomplete EDMs with the same number of missing ranges may result in two different rigid graphs after application of the same EDM completion algorithm. See Figure \ref{fig:edm-ambiguity}, where one incomplete EDM renders correct rigid graph whereas the other one does not, although both will take equal amount of time due to equal number of edges. This signifies the importance of edge selection f
or ranging to ensure fast and accurate  localization.

\begin{comment}
%
\subsection{Overview of Solution}
%localization
The localization problem is to determine the location (coordinate in 2D) of each entity in a global coordinate system, given the distances (ranges) between them, measured using wireless modality. We represent the entities as nodes in a graph. Each of $n$ nodes has a unique node ID labeled 1 through $n$. The length of the edge between two nodes correspond to the measured range between the two entities. 
%approach to solve the problem
When all the nodes are mobile, we solve the localization problem on a snapshot basis as follows. 
Given $n$ nodes, we have $^nC_2$ possible ranges, from which we construct a unique  geometric shape called rigid graph. The location of a node in this rigid graph is called relative location and the process is called relative localization. This rigid graph, however, can be rotated, translated or flipped with respect to any arbitrary coordinate system.
So, using additional information, we  fix the rigid shape with respect to a global coordinate system and thus derive unique absolute location of each node. This is called absolute localization. In other word, the solution in absence of fixed static anchor locations, involves relative localization followed by absolute localization.

%all-pair ranges impractical
In relative localization step, the objective is to determine the rigid graph as accurately as possible using the measured ranges. If all the $^nC_2$ ranges are measured accurately, we do derive a unique rigid graph \cite{rigid-geometry}. However, each measurement takes some finite amount of time, which cannot be minimized due to system constraint arising out of the wireless modality. For applications dependent on the real-time location of potentially mobile nodes, the objective is to localize each node repeatedly as fast as possible. However, even for a small number of nodes, say $n=16$, and for the ranging time  of say 40 msec, relative localization involving all possible ranges would take $^{16}C_2\times40/1000 =4.8$ sec. Within these few seconds, some highly mobile nodes will move to  new locations, which would  cause high localization error and would result in unsatisfactory performance of the dependent application. Moreover, some pairs of nodes may be out of each others wireless range, so range measurement is not possible for them. Either way, this ``all pair" range measurement is not practical. Therefore, the main challenge of relative localization is to determine the rigid graph as fast as possible by using least number of measurements (say 3$\times$16=48 ranges in 48$\times$40/1000 $=$ 1.92 sec instead of $^{16}C_2=$120 ranges in 4.8 sec). The natural question is - which edges to select for ranging.
%
%incomplete EDM, why? fast-refresh rate desirable, no physical links
To concertize the notion of edge selection as described above, we present the all-pair ranges between $n$ nodes, as an $n \times n$ matrix $\mathbf{D}$ called Euclidean Distance Matrix (EDM), where entry for row $i$ and column $j$ is the range between node $i$ and $j$. A compete EDM matrix gives unambiguous rigid graph. However, if we measure a subset of all-pair ranges, the resulting EDM will be incomplete i.e. the EDM will have missing values. An incomplete EDM does not guarantee a rigid graph. In literature, there are many ways to fill in the missing values  of a given incomplete EDM \cite{edm-completion}. However, in our case, the controller can choose which ranges to measure and thereby also the incomplete EDM. Note that, even if we apply the same matrix completion algorithm,  two different incomplete EDM with the same number of missing entries will result in two completely different rigid graphs as shown in Figure \ref{fig:incomplete-edm}. This ambiguity in rigid graph, defeats the whole purpose of relative localization, wherein we intend to determine the rigid graph uniquely for unambiguous localization. Therefore, an important challenge of relative localization is to determine which entries in the  EDM are crucial for determining unambiguous rigid graph formation. We also need to take into account the geometric dilution of precision (GDOP) \cite{gdp-paper} in determining this importance. Even if the measurements errors are low, the relative localization can incur huge error due to GDOP resulting from poor choice of the edges as shown in Figure \ref{fig:gdp}. 

%
Apart from the geometric requirement,
noisy entries of the EDM can also affect accuracy of rigid graph formation. This noise manifests in two ways i) node mobility and ii) channel characteristics. As for node mobility, between successive measurements, the range  between two static nodes remain unchanged whereas the range between two highly mobile nodes may change drastically. This change will result in temporal inconsistency in localization as shown in Figure \ref{fig:temporal-inconsistency}, where mobile nodes will contribute more to the localization error than static nodes. Therefore, it is desirable to range edges incident with highly mobile nodes more frequently than those incident with static nodes over time. In other word, the edge selection should also incorporate the expected node mobility. As for the channel characteristics, due to multi-path effect, some of the NLOS links will result in poor ranging accuracy compared to the LOS links. Therefore, existing channel characteristics should also be taken into account when selecting edges for ranging. 

In summary,  accurate and fast localization in our case is tied to accurate and fast formation of the rigid graph in the relative localization step. This involves i) deriving an incomplete EDM satisfying  the geometric requirements (rigidity and GDOP) and using high-accuracy ranges (based on node-mobility and channel characteristics), ii) deriving the complete EDM from the incomplete one and solving it for relative localization. \\
%
%
\end{comment}z
%method-intro
We start with an overview of our solution and then discuss each component of it.
%
\begin{figure}
\centering
\includegraphics[width = 0.99\linewidth ]{figs/flow.png}
\vspace{-0.1in}
\caption{Overview of our algorithm}
\label{fig:flow}
\vspace{-0.1in}
\end{figure} 
%
Figure \ref{fig:flow} shows an overview of the steps involved in our solution. The steps are i) Edge Selection ii) Ranging iii) Missing Range-estimation iv) Relative Localization and v) Absolute Localization. These steps are continuously repeated and the locations are fed into the applications as discussed in Section \ref{sec:applications}. Additionally, time-varying information about existing link quality and node mobility are collected periodically and used in these steps. Absolute localization also requires information beyond ranging. We discuss each step in detail in the order they are executed.
%
\subsection{Edge Selection}
As discussed in Section \ref{sec:background}, the ranging time cannot be arbitrarily minimized due to system constraint. Therefore, the goal is to repeatedly update the locations using least number of ranges. The edge selection step involves deciding which of the all possible links ($^nC_2$ for $n$ nodes) to range at the current instant for localization.
In particular,  we want to schedule ranging only for i) currently existing physical links, ii) links that are important for localization  iii) links that are incident with highly mobile nodes rather than static nodes, and iv) links with better channel characteristics and thus potentially better ranging accuracy. We now discuss measures involved in this step to ensure each of the above four objectives.
%

\subsubsection{Link Discovery}
The controller periodically broadcasts a  special discovery frame. Upon receiving this frame, each node sends out a beacon frame in the $i$-th TDMA slot where $i=1, 2,\ldots, n$ is the node ID. Each node upon receiving the beacon frame, adds the source node to its list of neighbors. The controller then collects the neighbor list from each node to build physical connectivity graph  $G(t) = (V, E(t))$ at instant $t$, where $V$ is the set of nodes and $E(t)$ is the set of existing links. In the following steps, ranging is only scheduled for the links in $E(t)$ instead of all $^nC_2$ possible ones. 
%
%
\begin{figure}
\centering
\includegraphics[width = 0.8\linewidth ]{figs/rigidity-example.png}
\vspace{-0.1in}
\caption{(a) Clique (rigid) (b) non-clique (rigid) (c) 2 choices for node 5 (not rigid) }
\label{fig:rigid}
\vspace{-0.1in}
\end{figure} 
%
\subsubsection{Determining Essential Links}
In this step, we determine the links that are important for localization. The importance is determined from two perspectives i) relative geometry- wherein the edges which are required to form unambiguous geometric shape (which we term rigid graph) from the ranges, are prioritized, and ii) node mobility- wherein the edges incident with relatively mobile nodes are prioritized. First, we describe how to resolve the geometric shape from scratch, which is required when the system starts up. We then present algorithm to incrementally update the shape using node mobility. To this end, we introduce the notion of rigid graph. 
%
\vspace{0.01in}
\\ \noindent
\uline{Rigid Graph:} 
Given a weighted graph $G=(V, E, d)$, where $d$ is the set of ranges of the edges, a \textit{realization} is a function $x:V \rightarrow{} \mathbb{R}^2$ that maps the set of vertices $V$  to 2D Euclidean space such that each range is preserved i.e $\forall (u,v) \in E, \; ||x(u) - x(v)|| = d(u, v)$ where $||.||$ is the Euclidean norm.
%
The graph $G=(V, E, d)$ is ``rigid" if there is only one realization discounting translation, rotation and flip. As shown in the Figure \ref{fig:rigid}, the complete graph or clique in (a) is rigid because given the 10 ranges between all  pairs of nodes, this graph is the only realization, although it can be rotated, translated and/or flipped. Similarly, given the 9 ranges, the graph in (b) is rigid. However, given the 8 ranges, as shown in (c), there are two choices to fix node 5 relative to the edge (2,3) resulting in  two realizations, therefore, it is not rigid.
%
We can define the following recursive definition of a rigid graph in 2D:
\begin{enumerate}[noitemsep, topsep = 0em]
    %
    \item A complete graph or clique is a rigid graph.
    %
    \item If $G=(V,E)$ is a rigid graph and a node $i$ has a set of edges $E_i$ to at least three non-collinear nodes in $G$, then the graph derived after adding node $i$ to the graph along with the connecting edges, is also rigid, i.e. $G^{'}=(V^{'},E^{'})$ is rigid, where $V^{'}=V\cup \{i\}$ and $E^{'}=E \cup E_i$.
 \end{enumerate}  
%
For example, the subgraph containing nodes 1 through 4 in Figure \ref{fig:rigid}(c) is rigid and all nodes are non-collinear. If we add an extra range (4,5), then node 5 becomes part of the rigid graph as shown in (b).
%
Using the above definition, we can incrementally build a rigid graph from the connectivity graph derived in the previous step, except  we need to know the ranges to determine collinearity. Therefore, we have a cyclic dependency as follows- the minimal rigid graph minimizes the required \# of ranges, yet determining the rigid graph requires knwoing the ranges. To this end, we introduce the notion of k-core graph to opportunistically range as the rigid graph is being built.
%
%
\vspace{0.05in}
%
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.8\linewidth ]{figs/k-core-example.png}
\vspace{-0.1in}
\caption{3-core Decomposition}
\label{fig:k-core-examples}
\vspace{-0.1in}
\end{figure}
%
\vspace{0.01in}
\\
\noindent \uline{k-core Decomposition}: A k-core is a connected  graph in which every node has a degree of at least k. For, $k\leq2$, the graph cannot be rigid in 2D. As shown in Figure \ref{fig:k-core-examples}, the connectivity graph  has 7 nodes, however, only nodes 1 through 4 can form a rigid graph.
%
Therefore, we try to find the rigid graph only on the $3$-core graph. In other words, the edges in the $3$-core graph are more important to range than the rest.
We specially handle the nodes in the $2$-core or $1$-core later. 
%
 Partitioning a graph into k-cores for $k=1,2,3,\ldots$ is called ``k-core decomposition". It works as follows. First the nodes with the lowest degree are removed one by one and are included in the k-core, where k is the degree during its removal. Such node-removal affects degrees of other nodes, so  the operation is repeated. The intra-core edges are preserved. As shown in Figure \ref{fig:k-core-examples}(a), nodes 6 and 7 have the minimum degree of 1, so both belong to 1-core. After removing them, we derive the 2-core subgraph in Figure \ref{fig:k-core-examples}(b). We then remove the  2-degree node 2, to derive the  3-core subgraph in Figure \ref{fig:k-core-examples}(c).
 %
 The 3-core decomposition does not require any ranging. It requires the connectivity matrix which is already determined in the previous step. Therefore, this step precedes rigid graph formation which requires ranging. We present two versions of rigid graph formation- i) bootstrap rigid graph formation: we compute the rigid graph from scratch when the system starts up ii) rigid graph update: based on the update in connectivity, 3-core graph and node mobility model, the existing rigid graph is updated. We briefly discuss them in the following.
 %
 \\
 \noindent \textbf{1. Bootstrap Rigid Graph Formation: }
 To maximize the chance of being part of the rigid body, we first rank the $m$ nodes in the 3-core subgraph according to the non-increasing value of their degree (degree in 3-core, not in the connectivity graph). Let the ordering be $n_1, n_2, \ldots, n_m$, where node $n_1$ has the highest degree. We start with the triangle (rigid graph) $<n1, n2, n3>$. It requires 3 ranges for the 3 sides of the triangle. From the connectivity matrix, we check whether node $n_4$ has edges with the above 3 nodes. If so, we measure 3 more ranges between them $n_4$ and the above 3 nodes. If the rigidity conditions are satisfied, we add $n_4$ to the triangle to form the new 4-node rigid graph. Then we try the next node $n_5$ and so on. The maximum number of ranging in this step equals the number of edges in the 3-core subgraph.
 %
 \\
 \noindent \textbf{2. Rigid Graph Update: }The new rigid graph $G_R(t+1)$  is derived from the existing rigid graph $G_R(t)$ by node deletion and addition. If there is a change in the connectivity graph (which is also continuously updated), the 3-core is recomputed. We first remove the nodes which fail the rigidity test in $G_R(t)$, due to the change in their connectivity. Removal of one or more nodes may cause  other nodes to be removed from $G_R(t)$. This way, we derive a smaller rigid graph $G^{'}_R(t)$ from $G_R(t)$. We then make a set of candidate nodes $V_c(t+1)$ for addition to $G^{'}_R(t)$ after rigidity test. The set $V_c(t+1)$ includes two types of nodes i) nodes which are in the updated 3-core graph but not in $G^{'}_{R}(t)$ and ii) nodes selected by the mobility model discussed later.  We start with a  node $n_i \in V_c(t+1)$ which has 3 edges to any three non-collinear nodes in $G^{'}_{R}(t)$, we measure the 3 ranges, make $n_i$ part of the rigid body by updating $G^{'}_{R}(t)$ and try another node in $V_c(t+1)$. After all nodes are tested, we derive the new rigid graph $G_R(t+1)$ from $G^{'}_{R}(t)$.
 %
 The maximum \# of ranging done in this step is  $3\times{}|V_c(t+1)|\leq$ \# of ranges required for rigid graph formation as in the bootstrap step.
  %
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.99\linewidth ]{figs/mobility-model.png}
\vspace{-0.2in}
\caption{Modeling of Uncertainty for a static and a mobile node}
\label{fig:mobility-model}
\vspace{-0.1in}
\end{figure}
%
 \vspace{0.01in}
 \\
 \noindent \uline{Mobility Model}: In the above, we handle the change of the rigid graph when nodes break away from it or new nodes become part of it due to change in connectivity. However, without change in connectivity, the rigid graph can also change due to the mobility of its existing nodes. In this section, we describe our approach to handle change in rigid graph due to node mobility. To this end, we define an uncertainty function $u_i(t)$ for each node $i \in V$ at instant $t$ which gives a distance measure of the uncertainty due to the elapsed time since the last localization of node $i$. We also set a threshold called tolerance of uncertainty denoted by $\Delta u$ and try to ensure that at any instant $t$, $\forall i \in V, \; u_i(t) < \Delta u$. The nodes are queried occasionally for their instantaneous linear velocity reading from the IMU. If the velocity is 0, the node is static and we define $u_i(t)$ by an exponential function $ab^{c\Delta t}$ where $\Delta t$ is the elapsed time since the last query for velocity and parameters $a,b$ and $c$ are chosen in accordance with $\Delta u$. In Figure \ref{fig:node-mobility}, the curve for the function $u_i(t)$ is shown for static node. The value of $u_i(t)$ keeps increasing  until node $i$ is localized (at 500msec and 1000msec marks) and we reset it to zero and then again increase it exponentially. As for a mobile node, when we derive a non-zero velocity $v_1$ from the IMU at instant $t_1$, we update the function as $u_i(t) = u_i(t_1)+v_1(t-t_1)$ (See 500msec mark). 
 %If the velocity is found to be $v_2$ at $t=t_2$, we update the function as $u_i(t) = u_i(t_2)+v_2(t-t_2)$ and so on. 
 If at $t_2$ node $i$ is localized and velocity is determined to be $v_2$, we reset the function as $u_i(t) = v_2(t-t2)$ (See 650msec mark). In other words, the uncertainty is modeled on the observed node velocity which is not used in the localization, rather is used as a measure for localization priority for nodes. The uncertainty keeps increasing until the node is ranged and localized. We maintain a priority queue for all nodes based on their current uncertainty  values. We always choose the highest priority node for the rigidity test and subsequent computation for localization. In this way, locations for relatively mobile nodes are more frequently updated than those for the static ones and our system is able to handle heterogeneous node mobility. 
 %
 %\textcolor{blue}{discuss function $u_i(t)$ in terms of IMU input}
\subsubsection{Link Quality Metric}
 %
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.95\linewidth ]{figs/linkq.png}
\vspace{-0.2in}
\caption{Factors of link quality metric shown in amplitudes of IQ-samples}
\label{fig:linkq}
\vspace{-0.1in}
\end{figure}
%
 %
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.8\linewidth ]{figs/linkq-validate.png}
\vspace{-0.2in}
\caption{LQ values and ranging errors for varying true distances}
\label{fig:linkq-validate}
\vspace{-0.1in}
\end{figure}
%
%necessity of linkq quaity metric, refer to background
When all the nodes are closer to each other, the available links for ranging are often more than the required 3 links per node for the  rigid graph formation.  As discussed in Section \ref{sec:background}, one or more ``poor quaity" links can deteriorate the accuracy of the ranging and thereby, the accuracy of the resulting localization. Therefore, these links should be ordered according to a quality metric which reflects the probability of ranging error, and the best 3 links should be selected.
%
In our system, each node maintains a list of Link Quality (LQ) metric value, one for each other node. Each LQ value is initialized as zero (indicates no wireless link). The LQ value is updated whenever a frame is received due to either overhearing or the node being the destination. We assume that this LQ value holds momentarily due to potential node moblity, therefore each LQ value is reset to zero in every few seconds after the last update. We now discuss the formulation of the LQ values. 

In our system, the UWB chip Decawave DW1000\cite{deca1000},  calculates the range based on the finegrained timestamp of  the firstpath detection. The ranging error (always a positive bias) originates mostly due to the erroneous detection of the firstpath.
The detection algorithm is proprietory, however, the chip saves the set of IQ samples on which the anaysis is done after each frame reception. Depending on the operating mode selected for the UWB chip, the number of 4-byte IQ samples is  about between 1K and 4k.
Collecting kilobytes of IQ sample from the UWB chip in submillisecond after every frame-reception is not feasible due to relatively slow microcontroller (72MHz STM32F series \cite{stm32}). It can also be disruptive to ongoing ranging operation as the UWB chip has to switch between TX and RX mode on demand without getting stuck in the LQ calculation. Therefore, we compute the LQ metric based on the few frame quality values saved in UWB chip registers after every frame reception in a manner non-disruptive to the ongoing ranging operation. The LQ value for the link between node $i$ and $j$ is defined as follows:
\begin{equation}
LQ(i, j) = f_1 \times{} f_2 \times{} f_3 \times{} f_4
\label{eq:linkq}
\end{equation}
Here, the 4 factors are defined as follows:
\begin{enumerate}[noitemsep, topsep = 0em]
    \item \textit{Inverse of avg. peak-count in the preceeding window ($f_1$)}: This is the inverse of the average number of peaks (defined by a rising value followed by a falling value) in a small (typically 6 samples) window of amplitudes preceding the the first-path (FP). Each peak must be $>$ the Standard Deviation (STD) of the noise (constantly calculated by the chip).  As shown in Figure \ref{fig:linkq}, FP is marked by red and the std noise is marked by the dotted horizontal line. Here, the peak count is 1, window size is 6 (3 peaks possible), hence avg. peak count is 1/3 and $f_1=\frac{1}{0.005+1/3}=2.955$. Here, a small constant $0.005$  is used to circumvent divide-by-zero error. The lower the number of peaks, the higher the chance of accurate FP detection, and the higher the value for $f_1$.
    \item \textit{FP to STD-noise amplitude ratio ($f_2$)}: The UWB chip updates the standard deviation of noise (STD-noise) during each frame reception. We take $f_2$ to be the ratio between FP amplitudue and STD-noise amplitude. This value is in dB. The higher the ratio i.e. $f_2$, the more prominent the FP is and the higher probability of accurate FP detection.
    \item \textit{ FP to peak amplitude ratio ($f_3$)}: This is the ratio between the FP amplitude and the peak or maximum amplitude in the entire sample. In most LOS cases (high quality ranging), the FP is often the peak amplitude. Therefore, the higher the ratio i.e $f_3$, the more accurate is the ranging value.
    \item \textit{ Ratio between the FP power and the total received power ($f_4$)}: This ratio is also indicative of the prominance of the FP. In LOS cases, the ratio in dB is significantly higher than the NLOS cases. Hence, higher the value for $f_4$, the the more accurate is the range value.
\end{enumerate}
All the four factors defined above are ratios i.e. unit-less values. Therefore, LQ is unitless and its high value is indicative of less erroneous ranges. The computation is simple and requires only few tens of bytes to be  read from the registers of the UWB chip, therefore can be done in the microcontroller attached to the UWB chip in submillisecond. 
%

To validate the LQ metric, we put a pair of UWB transceivers in LOS and NLOS conditions at various distances and collect the true distance, computed range and the corresponding LQ value. We take the error to be the difference between the true distance and the computed range. We then plot the average error and the avg. LQ values against corresponding true distances for diverse scenarios as shown in Figure \ref{fig:linkq-validate}. Here, the LQ value is inversely proportional to the ranging error. Also notable is the gap between NLOS and LOS both for ranging error and metric value. For NLOS case, nodes could not be ranged beyond 20 meters in extreme indoor multipath environment.

%
 \subsubsection{Summary of Edge Selection}
%
\begin{algorithm}[htb!]
%
\caption{Edge Selection in Controller}
\label{algo:edge-selection}
\begin{algorithmic}[1]
  %\scriptsize
   %
  \STATE Initialize rigid graph $G_R = \varnothing$, link matrix $\mathbf{L}$, mobility matrix $\mathbf{U}$ 
  %
  \FOR{each node $i\in V$}
    \STATE Command node $i$ to transmit beacon frame
  \ENDFOR
%
  \WHILE{\textbf{True}}
    %
    \FOR{each node $i\in V$}  
        \STATE Collect link quality and velocity from node $i$
        \STATE Update matrix $\mathbf{L}$ and $\mathbf{U}$
    \ENDFOR
     %
     \STATE Purge nodes from $G_R$ after rigidity test 
     \STATE Compute 3-core graph $G_3$ 
     \STATE $V_c \xleftarrow{} \{i | i \in G_3 \mbox{ and } i \not\in G_R\}$
     \STATE $V_c \xleftarrow{} V_c \cup \{ {\underset{i}{\arg\max} \; \mathbf{U}} \}$  
     \REPEAT 
        \STATE $i \xleftarrow{}$ highest degree node from $V_c$
        \STATE $E_i \xleftarrow{}$ edges between $i$ and $G_R$
        \IF{Node $i$ and graph $G_R$ is rigid }
            \STATE $E^{'}_{i} \xleftarrow{}\{ {\underset{e_1, e_2, e_3 \in E_i}{\arg\max} \; \mathbf{L}(E_i)} \} $ 
            \STATE \textbf{Collect ranges} for edges in $E^{'}_i$
            \STATE Add $i$ to $G_R$ by edges in $E^{'}_i$
            \STATE $V_c \xleftarrow{} V_c - \{ i \}$ 
        \ENDIF
     \UNTIL{no node $i \in V_c$ can be added to $G_R$}
    \STATE  \textbf{compute relative locations}
  \ENDWHILE
\end{algorithmic}
%
\end{algorithm}
 %
 We can summarize the steps in edge selection in Algorithm \ref{algo:edge-selection}. Line 1 through 4 are part of the bootstrap step. We start with empty rigid graph $G_R$, initialize the $n\times{}n$ zero matrix as link quality matrix $\mathbf{L}$ and initialize mobility model $\mathbf{U} = [u_1(t) \;\; u_2(t)\;\; \ldots u_n(t)]^T$. Operations from Line 5 through 25 are repeated continuously for relative localization. In each round, link quality and mobility matrices are updated (See Line 5 through 9), then rigid graph is updated based on their updated values (See Line 10 through 23). Finally, relative locations are calculated in Line 24 which is discuss later. Note that, we only measure ranges in Line 19. The purpose of this algorithm is to minimize this measurement yet achieve high accuracy localization. We now present the details of this ranging operation. 
 %
 \subsection{Ranging}
   %
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.99\linewidth ]{figs/twr.png}
\vspace{-0.1in}
\caption{Different Ranging Protocols}
\label{fig:twr}
\vspace{-0.1in}
\end{figure}
%
In this section, we describe the ranging operation and related protocol in detail. We start by briefly describing the two-way ranging protocol and its optimization. We then discuss frame format, its payloads and other system parameters associated with ranging operation.
%
\\ \noindent \textbf{Two-way Ranging (TWR):}  We can calculate the range between two nodes from the TOF of a single frame between them. However, it requires both their clocks to be precisely synchronized which is not practical in our setting. Two-way ranging protocol as shown in Figure \ref{fig:twr}, does not require clock synchronization. The simplest and quickest version of TWR is the Single Sided TWR (SS-TWR) where two frame named ``poll" and ``response" are exchanged to calculate TOF. However, there are a number of sources of error due to clock drift and frequency drift \cite{twr}. To minimize the error, one extra frame named ``final" is exchanged and it is called Double Sided TWR (DS-TWR) as shown in Figure \ref{fig:twr}. Calculating  the intervals $D1$, $R1$, $D2$ and $R2$  from the tx/rx timestamps of these three frames, we can calculate the TOF as $\frac{D1\times{}D2-R1\times{}R2}{2\times{}(D1+R1)} = \frac{D1\times{}D2-R1\times{}R2}{2\times{}(D2+R2)}$. Both values should be close and an average of them is taken as TOF. When node 1 ranges with more than 2 nodes, it can run DS-TWR sequentially with them (SEQ-DS-TWR in Figure \ref{fig:twr}). We introduced an extra frame called ``Init" (for initialization) that triggers the ranging. The Init frame also carries additional information about the parameters of ranging that we describe later. Also, due to Init frame, the pairwise ranging operation finishes with node 1 instead of node 2 or 3 and the initiator node 1 is able to calculate the range. Note that, the tx timestamp of the poll and final (pre-calculated \footnote{Once the frame is scheduled for tx, the tx-timestamp can be calculated from the antenna delay even before the acutal tx}) frames and the rx timestamp of the response frame embedded in the Final frame as data so that the initiator node can calculate the TOF without any further frame exchanges.
Altogether, this operation takes 4 TDMA slots per ranging pairs. However, we can save slots by making the common node 1 to transmit all frames (Init and Response frames) only once. This way, two slots are saved per nodes. For example if a node ranges with $n$ nodes, instead of $4n$ slots, it will require $2+2n$ slots (6 slots instead of 8 in the example in Figure \ref{fig:twr}). We term this protocol Optimized Double Sided TWR (OPT-DS-TWR). Here, the initiator node will embed the slot time, response order of the nodes etc in the Init and Response frames, and the participating nodes follow the order in sending the Poll and Final frames. 
 %
%
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.99\linewidth ]{figs/forwarding.png}
\vspace{-0.1in}
\caption{Alternate Data Forwarding Methods}
\label{fig:forwarding}
\vspace{-0.1in}
\end{figure}
%
%\textcolor{blue}{ Discuss frame structure, piggybacked data, TDMA slot time, wifi out of band communication etc.}
\\ \noindent \textbf{Data Forwarding:} Collecting ranges, mobility and link quality information etc. from the nodes also adds up to the localization delay. We have two choices- in-band and out-of-band data forwarding as shown in Figure \ref{fig:forwarding}. In in-band strategy,
we use the UWB links to transfer the data via a forwarding tree rooted at the controller node as shown in Figure \ref{fig:forwarding}(a). However, due to the limited ranging of UWB, some of the nodes may be disconnected form the controller (no path between Node 1 and 3 etc). Also, this does not scale up well with increasing \# of nodes and increasing node mobility due to the constant overhead of maintaining the forwarding tree. Note that, there may be rigid subgraphs which otherwise be relatively localized yes does not have a path to the controller node. The other strategy is out-of-band modality such as WiFi, LoRa etc. that fully covers the area of interest. This way, each node can directly forward data frame to the controller node, as shown in Figur \ref{fig:forwarding}(b). 
In our system, we used WiFi-long-range (range of 100 meter indoor) since WiFi is ubiquitous, inexpensive, has higher data-rate and can itself be used for ranging in case UWB links fail for sustained period of time, although WiFi ranging is less accurate than UWB (discussed in Section \ref{sec:fail-safe}).
 %
 %
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.9\linewidth ]{figs/frame.png}
\vspace{-0.1in}
\caption{UWB Frame Format}
\label{fig:frame}
\vspace{-0.1in}
\end{figure}
%
 \\ \noindent \textbf{Data Frame:} The controller directs a particular node $i$ for ranging with a list of nodes via WiFi. This WiFi packet also contains UWB slot-time which is calculated precisely using UWB data-rate and maximum UWB frame-size. By not using a fixed-slot time for all cases, our system can dynamically adapt to the existing \# of nodes. After reception of the WiFi frame, the node initiates the OPT-DS-TWR protocol immediately with the list of nodes. In particular, the Init frame contains the list of nodes plus the slot time. After ranging is done, Node $i$ sends the ranging data along with i) velocity and heading data (discussed in Section \ref{sec:abs}) from IMU and ii) current link quality values of existing links. Moreover, all participating nodes in the ranging, also piggybacks their velocity,  heading and link quality values over the UWB frame i.e via Poll and Final frames. We re-purposed IEEE 802.15.4-2011-UWB frame for Init, Poll, Response and Final frames which carry the information, as shown in Figre \ref{fig:frame}. This way, the controller can get mobility and link quality data as part of continuous ranging, which eliminates Step 6 through 9 in Algorithm \ref{algo:edge-selection}. Since, 2-way WiFi communication takes at least few milliseconds, for tens of nodes, the saving is hundreds of milliseconds in the main loop of the algorithm. In the frame format (See Figure \ref{fig:frame}, the Frame Control (FC) byte distinguishes our custom IEEE-802.15.4 frame. It is followed by sequence-\#, Personal Area Network (PAN ID), source and destination ID\footnote{1-byte source and destination ID supports 256 nodes, which we assume, is sufficient for all indoor deployments}, Function Code (FCode) (indicates frame type- i.e whether Init, Poll etc.), variable-byte payload and and 2-byte Frame Control Sequence (FCS). Mobility, link quality and timestamp information (40 bit each) for ranging are embedded onto the payload. Due to limited data-rate of UWB link, this simplified and reduced frame-format minimizes required slot time and thereby, the ranging time.
 %
 \subsection{Missing Range Estimation \& Relative Localization}
 %
 %\textcolor{blue}{Discuss EDM, its loss function, estimation of its missing values via FloydWarshall shortest path method, solving EDM by Classic Multidimensional Scaling, EDM calculation interval based on loss function update, adding 2-core and 1-core nodes to the rigid graph}
 %
 %
 %
 Once the rigid graph has been formed for $n$ nodes, we derive $n\times n$ the Euclidean Distance Matrix (EDM) $\mathbf{D}$ where each entry in row $i$ and column $j$ is the distance between node $i$ and $j$. We then  try to solve it for relative locations using a widely known technique known as Classical Multi-Dimensional Sampling (CMDS) that we now briefly introduce. We also justify our choice in the following.
%
\\ \noindent \textbf{Classical Multi-Dimensional Sampling (CMDS) Problem: }
Given a complete $n\times{}n$ matrix $\mathbf{D^2}$ of squared distances $d^2_{ij}$'s between node $i$ and $j$, CMDS problem is to find the $n\times{}d$ coordinate Matrix $\mathbf{X}$ that gives the location $\mathbf{x}_{i}$ of each node $i$ in $d$-dimensional Euclidean Space. In matrix notation, this amounts to solving for $\mathbf{B}=\mathbf{XX^T}$ where $\mathbf{X^T}$ is the transpose of matrix $\mathbf{X}$. As shown in \cite{cdms-paper}, $\mathbf{X}$ can be calculated as follows:
\begin{equation}
    \mathbf{D^2}=\mathbf{C\,1^T}+\mathbf{1\,C^T}-2\mathbf{XX^T}
    \label{eq-dsquare}
\end{equation}
Here, $\mathbf{C}$ is the $n\times{}1$ matrix with only the diagonal elements of $\mathbf{XX^T}$ and $\mathbf{1}$ is the $n\times{}1$ matrix of ones. By multiplying both sides of Equation \ref{eq-dsquare} by the centering matrix $\mathbf{J}=\mathbf{I}-\frac{1}{n}\mathbf{1\,1^T}$ and some algebraic manipulation, we have
%
\begin{equation}
 \mathbf{X} = \mathbf{Q}\sqrt{\Lambda}\mbox{ where } \mathbf{B}=\mathbf{Q}\,\Lambda\,\mathbf{Q^T}=-\frac{1}{2}\mathbf{JD^2J} 
 \label{eq:cmds}
\end{equation}
%
Therefore, CMDS algorithm involves the following 3 steps-
\begin{enumerate}[noitemsep, topsep = 0em]
    \item  Given square-distance matrix $\mathbf{D^2}$, compute Gram matrix $\mathbf{B}$ of $\mathbf{X}$ as $\mathbf{B}=-\frac{1}{2}\mathbf{JD^2J}$,
    \item Find the Eigenvalue decomposition of $\mathbf{B}=\mathbf{Q}\,\Lambda\,\mathbf{Q^T}$, 
    \item Finally, compute $\mathbf{X}=\mathbf{Q}\sqrt{\Lambda} $ for Eigenvector matrix $\mathbf{Q}$ and diagonal Eigenvalue matrix $\Lambda$.
\end{enumerate}
%
%
\begin{figure}[htb!]
\centering
\includegraphics[width = 0.99\linewidth ]{figs/cmds-adv.png}
\vspace{-0.1in}
\caption{Advantage of CMDS over sequential multilateration}
\label{fig:cmds-adv} 
\vspace{-0.1in}
\end{figure}
%
Due to the ``centering" assumption, each column of solution $\mathbf{X}$ sums to zero i.e, the origin of $\mathbf{X}$ coincides with the centroid of the $n$ locations. 
Note that CMDS minimizes the loss function (also called \textit{strain}) $L( \mathbf{X} ) = ||\mathbf{XX^T} - \mathbf{B}||=||\mathbf{XX^T} - \frac{1}{2}\mathbf{JD^2J}||$. As such, the CMDS can end up in local minima. These local minima is more likely to occur when dimension is low (2  as in our case) \cite{cmds-book}. Therefore, cross-validate the locations using heading data of nodes discussed in Section \cite{ref:heading-validate} and also run a smoothing filter on the successive node locations over a small window. CMDS has distinct advantage over using sequential multilaterion as shown in Figure \ref{fig:cmds-adv}. Here, 5 nodes form a complete graph as shown in Figure \ref{fig:cmds-adv}(a). We can use multilateration to fix node 4 using node 1, 2 and 3, then fix node 5 using 1,3 and 4. However, nodes mulitlaterated later in the sequence will incur prohibitively high localization error (shown in shaded circle). But CMDS solve the localization problem  by taking into consideration all the ranges (complete EDM) and jointly minimizing the loss function. In this way, no node ordering is required and localization error is not lumped into handful of nodes.
%
%
\begin{algorithm}[htb!]
%
\caption{EDM Completion Algorithm}
\label{algo:edm-completion}
\begin{algorithmic}[1]
  %\scriptsize
  %
  \STATEx \textbf{Input:} Weighted Graph $G = (V, E, d)$ where $V$ is the set of vertices, $E$ are edges with measured ranges $d$.
  \STATEx \textbf{Output:} Complete EDM $\mathbf{D}$
 %
  \STATE Initialize relative location matrix $\mathbf{X}$ using sequential multilateration 
  %
  \STATE Iteration count c $ \leftarrow 1$ 
  \WHILE{c$<$ Max. Iteration}
  \STATE $E_c \leftarrow \{(i, j)|i < j \mbox{ and }i,j \in V\}$
   \WHILE{$E_c \neq \emptyset$}
    \FOR{  $\forall(i, j)\in E_c$}
         \STATE $\Delta \mathbf{x}_{ij} \leftarrow \displaystyle{\frac{ | ||\mathbf{x}_i -\mathbf{x}_j|| - d_{ij} |  }{||\mathbf{x}_i -\mathbf{x}_j||} } \; (\mathbf{x}_i -\mathbf{x}_j)$
    \ENDFOR
   \STATE $(i, j) \leftarrow \displaystyle{ \underset{(i,j) \in E_c}{\arg\max} \;  \Delta \mathbf{x}_{ij}}$
   \STATE $\mathbf{x}_i \leftarrow \mathbf{x}_i + \lambda \Delta \mathbf{x}_{ij}/2$,  $\mathbf{x}_j \leftarrow \mathbf{x}_j - \lambda \Delta \mathbf{x}_{ij}/2$
    \STATE $E_c \leftarrow E_c - \{(i,j )\}$
  \ENDWHILE 
  \STATE Update each entry $(i,j)$ of $\mathbf{D}$ as $ d_{ij} = ||\mathbf{x}_i -\mathbf{x}_j||$
  \STATE  $\displaystyle {\lambda \leftarrow \frac{1}{1+c\Delta\lambda} }$
  \ENDWHILE
 %
\end{algorithmic}
%
\end{algorithm}
 %
%
\\ \noindent \textbf{EDM Completion: } In the rigid graph formation, some node may have only 3 edges. Therefore, the rigid graph is not necessarily a clique and a lot of edges remain to be measured. But CMDS requires a clique i.e. a  complete EDM, so we need to fill in the missing values. There are few ways to do it. We adopt EDM completion algorithm based on proximity adjustment \cite{confo-sampling} as shown in Algorithm \ref{algo:edm-completion}. 
%
Here, we take an arbitrary triangle on nodes $<i, j, k>$ from the rigid graph, arbitrarily consider i) location of node $i$ as the origin, ii) edge $(j, k)$ aligned along the positive x-axis, iii) location of node $k$ in the positive y-quadrant. Then we resolve relative locations for the rest of the nodes using sequential multi-lateration. 
%
Each node will get a relative location due to the already satisfied rigidity condition. Now, we want to improve EDM via successive updates based on the difference between the  distance $||\mathbf{x}_i - \mathbf{x_j}||$, derived using the current  locations for node $i$ and $j$  and the distance  $d_{ij}$ found in the current EDM $\mathbf{D}$. This change vector $\Delta \mathbf{x}_{ij}$ is applied to  locations of both node $i$ and $j$ as in Line 10 in Algorithm \ref{algo:edm-completion}. Note that $\lambda$ is the update-rate which decreases with iterations. We repeat the iterations by considering each edge once and updating $\mathbf{X}$ and then $\mathbf{D}$  and terminate the algorithm when improvement in successive iterations is negligible ($>$0.001\%) or when a max. iteration (computed from remaining time for localization) is reached. Once the full EDM is computed from the rigid graph, the CMDS algorithm is applied to derive the relative location matrix $\mathbf{X}$ according to Equation \ref{eq:cmds}.
%
\\ \noindent \textbf{Relative Locations for Excluded Nodes: } So far, we computed the relative locations for nodes which were part of the rigid graph. Now, we discuss technique to relatively localize nodes not part of the rigid graph. We categorize nodes in two types-  nodes having i) two edges and ii) only one edge with nodes of the current rigid graph. For 2-edge case, we have two candidate relative locations by solving the two distance equations, See  node 5  in Figure \ref{fig:rigid}(c). Out of the two, we choose the relative location using the link information of the candidate node and the proximity constraint. For example, in Figure \ref{fig:rigid}(c), node 5 detects links with node 2 and 3, but not with node 1 or 4. Therefore, we choose that location for which both distances $d_{1,5}$ and $d_{4,5}$ are of greater value. However, the 1-edge case is not geometrically solvable. However, we still use the single range the heading information derived from the IMU to determine the relative location of the node as discussed in the next section.  
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %
 \begin{comment}
 \subsection{Absolute Localization}
Given the relative location $\mathbf{x}$ of a node, we derive the absolute location by the  transformation $\mathbf{x}_{abs} = \mathbf{r}\mathbf{x}+\mathbf{t}$, where $\mathbf{r}$ and $\mathbf{t}$ are the $2\times{}2$ rotation matrix and $2\times{1}$ translation matrix respectively indicating the required rotation and translation of the coordinate of the relative locations. First, we discuss how to find the vectors using one fixed node. Then we discuss how to embed the rigid graph on a floormap.
%
\\ \noindent \textbf{Using One Fixed Node: } We assume that a fixed node works as the origin of the global coordinate system. Such a node can be placed at the entrance or any other known landmark of the indoor area.  If we take this particular node as the origin during rigid graph formation, then $\mathbf{t} =\begin{bmatrix} 
0 \\
0
\end{bmatrix}$. 
%
To determine the rotation angle $\theta$ for the relative coordinate,
we also assume that the earth's magnetic north-south axis aligns with the global y-axis. Under this scenario, we measure the headings (angle with earth's north-south axis) of any 2 mobile\footnote{We assume that when the nodes are mobile, the angle between the  direction of motion and the earth's north-south axis is constant for the time being. } nodes $i$ and $j$ as $\theta_i$ and $\theta_j$ and set $\theta =(\theta_j - \theta_i$) and  $\mathbf{r} = \begin{bmatrix}
\cos\theta & -\sin\theta \\
\sin\theta & \cos\theta
\end{bmatrix}$. Since the headings are noisy, we generally maintain a small window of past heading values for each node, take smoothed values to calculate $\theta$ and finally take average of all the $\theta$ values calculated for all pairs of mobile nodes. 
\\ \noindent \textbf{Embedding on Floormap: }
%
\end{comment}
\clearpage

==> method/2-relative-loc.tex <==
\begin{comment}
%\subsection{Relative Localization}
%\label{sec:relative-loc}
%subsec-intro 
In this section, we discuss the method to determine the relative geometry formed by the nodes. The first step is to range between pair of nodes to determine inter-node distances. As discussed in Section \ref{sec:time-constraint}, the naive approach i.e. making measurements for all possible pairs, does not take into consideration the dynamic topology of the connectivity graph, and takes prohibitively long time for localization. Therefore, we propose ``edge selection" algorithm based on factors such as channel characteristics, node mobility and geometric requirements. We discuss a novel protocol that enables this dynamic edge selection. Finally, we discuss ways to estimate the missing ranges in the above steps to unambiguously form the relative geometry.
%
%relative localization
%\subsubsection{Edge Selection}
%\label{sec:}
%The purpose of edge selection algorithm is to schedule ranging only for i) currently existing physical links, ii) links that are important to remove ambiguity in constructing the relative geometry,  iii) links that are incident with highly mobile nodes rather than static nodes, and iv) links with better channel characteristics and thus better ranging accuracy. In the following, we present our approach to achieve the above goals for edge selection by efficiently using each TDMA slot. Due to the changing connectivity over time due to node mobility and limited wireless range, we term the physical connectivity graph at instant $t$ as $G_c(t) = (V, E(t))$, where $V$ is the set of all edges and $E(t)$ is the set of existing edges.
%
%\\ \noindent \textbf{Bootstrapping:} When the system starts up, it has no knowledge about the node locations, physical connectivity etc. Therefore, in this bootstrap step, the focus is to gather information to build an initial state from which continuous localization can proceed. Bootstrapping involves the following steps-  i) Connection Discovery ii) K-core Decomposition iii) Rigid Graph Formation. 
\vspace{0.05in}
\\
%\noindent \textit{1. Connection Discovery}: After starting up, the controller  broadcasts a a special discovery frame. Upon receiving this frame, each node sends out a beacon frame in the $i$-th TDMA slot where $i=1, 2,\ldots, n$ is the node ID. Each node upon receiving the beacon frame, adds the source node to its list of neighbors. The controller then collects neighbor list from each node and builds up initial ( at iteration $t=0$ ) physical connectivity graph $G(0) = (V, E(0))$. 

%each node sends out a neighbor discover given $n$ nodes, it collects ranges for all possible pairs ($^nC_2$) of nodes. Due to frame-loss, some of the ranges may not be collected. Therefore, additional attempts are made to collect those missing rages. After few of such attempts, the system is able to build the physical topology along with the edge lengths. We term this graph as the initial physical connectivity graph $G(0) = (V, E(0))$ at iteration $t=0$. Any further computation of determining the locations is done incrementally on this graph.
%
%
%After collecting all possible ranges, the following two computations are done on graph $G(0)$ as part of the bootstrap step, i) $k$-core decomposition \cite{k-core} and ii) rigid graph formation for $3$-core. We first describe the steps as follows. 
%
\vspace{0.05in}
%
\begin{figure}
\centering
\includegraphics[width = 0.75\linewidth ]{figs/k-core-example.png}
\vspace{-0.1in}
\caption{K-core Decomposition Examples}
\label{fig:k-core-examples}
\vspace{-0.1in}
\end{figure}
%
\vspace{0.05in}
\\
\noindent \textit{1. k-core Decomposition}: A k-core is a maximal graph in which every node is connected to at least k other nodes. In our case, k-core indicates whether a subgraph can form a rigid graph or not. In particular, if k$\geq$3,  the subgraph has potential to be a rigid graph in 2D based only on the range measurements, otherwise not \cite{2d-geom}. As shown in Figure \ref{fig:k-core-examples}, the connectivity graph $G(0)$  has 7 nodes, however, only nodes 1, 2, 3 and 4 can form a rigid graph (described later) required for relative localization. Therefore, including ranges such (5, 6), (2, 5) etc. will not contribute to the relative geometry. Partitioning a graph into k-cores for $k=1,2,3,\ldots$ is called ``k-core decomposition". It works as follows. First the nodes with the lowest degrees are removed one by one and are included in the k-core, where k is the degree during its removal. Such removal affects other nodes and the operation is repeated until no nodes remain. As shown in Figure \ref{fig:k-core-examples}(a), nodes 6 and 7 have the minimum degree i.e 1 and both belong to 1-core. After removing them, we derive the graph as in Figure \ref{fig:k-core-examples}(b), where there is no 1-degree node. We then remove all 2-degree nodes and then all 3-degree nodes to derive 2-core and 3-core subgraphs (c) respectively.
%
\vspace{0.05in}
\\
\noindent \textit{2. Rigid Graph Formation}: After formation of 3-core subgraph $G_3(0)$ out of initial connectivity graph $G(0)$, the next operation is to form a rigid subgraph $G_R(0)$ from it. However, to determine rigidity, the edge-lengths or the ranges are required. Therefore, in this step, the controller collects ranges between all pairs of nodes ($^mC_2$ for $m$ nodes) in the 3-core graph. Rigid graph is formally defined in the following.

\begin{comment}
A \textit{realization} is a function that maps a given set of vertices to 2D Euclidean space. Given a simple, connected, weighted graph $G=(V, E, d)$, where $V$ is the set of vertices, $E$ is the set of edges and $d(u, v)$ is the Euclidean distance or range between nodes $u, v \in V$,  the DGP problem is to find whether there is a realization $x:V \rightarrow{} \mathbb{R}^2$ such that each range is preserved i.e $\forall (u,v) \in E, \; ||x(u) - x(v)|| = d(u, v)$ where $||.||$ is the Euclidean norm.
\end{comment}
\begin{comment}
\\ \noindent
\uline{Rigidity Graph:} 
Given a connected and weighted graph $G=(V, E, d)$, where $d$ is the set of ranges of the edges, a \textit{realization} is a function $x:V \rightarrow{} \mathbb{R}^2$ that maps the set of vertices $V$  to 2D Euclidean space such that each range is preserved i.e $\forall (u,v) \in E, \; ||x(u) - x(v)|| = d(u, v)$ where $||.||$ is the Euclidean norm.
%
The graph $G=(V, E, d)$ is ``rigid" if there is only one realization discounting translation, rotation and flip. As shown in the Figure \ref{fig:k-core-examples}(c), subgraph $G_3(0)$ in (c) is rigid, but $G_2(0)$ in (b)  is not, because given the ranges for edge (2, 5) and (4, 5), node 2 can be placed in two locations relative to edge (2, 4). These two realizations are not rotation, translation or flip of each other. Similarly, 1-core subgraph i.e. the connectivity graph $G(0)$ is not rigid. We can define the following recursive definition of a rigid graph in 2D:
\begin{enumerate}[noitemsep, topsep = 0em]
    %
    \item A complete graph or clique is a rigid graph.
    %
    \item If $G=(V,E)$ is a rigid graph and a node $i$ has a set of edges $E_i$ to at least three non-collinear nodes in $G$, then the graph derived after adding node $i$ to the graph along with the connecting edges, is also rigid, i.e. $G^{'}=(V^{'},E^{'})$ is rigid, where $V^{'}=V\cup \{i\}$ and $E^{'}=E \cup E_i$.
 \end{enumerate}  
%
Condition 2 above requires each node to have degree 3 i.e. the graph has to be 3-core. But this is not a sufficient condition, we also need to test collinearity of the 3 nodes connecting each node in the subgraph. As such, rigid graph is a subgraph of 3-core graph. The 3-core in Figure \ref{fig:k-core-examples}(c) satisfies this condition, therefore it is rigid. If we add edge (5,1) and or (5,3) to the connectivity graph, then node 5 also becomes part of the rigid graph by the above conditions. For a given 3-core, we can start with an arbitrary edge or triangle (a clique) and try to add nodes following the above conditions to form a rigid graph $G_R(0)$. Overall, after collecting all possible ranges in the bootstrap step, we can summarize the derivation as $G(0) \Rightarrow{} G_3(0) \Rightarrow{} G_R(0)$. Nodes not part of the rigid graph $G_R(0)$ requires additional information for localization discussed later. Once, remaining nodes are added to $G_R(0)$ using additional information such as heading from IMU etc, we derive augmented rigid graph $G_R^{'}(0)$ and from it, the absolute locations of each node as described in Section \ref{sec:abs-loc}.

\uterm{Incremental Update} After bootstrapping, all computations are incremental to the initial rigid graph $G_R(0)$ derived in the previous step. In particular, we derive the rigid graph $G_R(t+1)$ from $G_R(t)$ for iteration $t=1,2,\ldots$etc. There are two steps in the incremental computation as described below.
%
\\ \noindent \textit{1. K-core Update}: Due to the broadcast nature of wireless communication, each node overhears transmissions within its communication range and determines the source node ID from the received frame. These overheard nodes are the neighbors in the connectivity graph. Each node maintains a list of overheard neighbors along with the timestamps. The nodes that have not been overheard for long time are purged from the list.
At each iteration $t$, the neighbor list of each nodes are collected to form the connectivity graph $G(t)$. Then k-core decomposition is computed on it to derive 3-core graph $G_3(t)$. Note that, this step does not require any ranging.
%
\\ \noindent \textit{2. Rigid Graph Update}: This step requires ranging to update the rigid graph. To miin
%protocol design
\end{comment}

%edm completion



==> old-method.tex <==
%method
\label{sec:method}
%IMU cross validation
%\section{Relative Localization}
In Rigid body formation, given the set of range $R$, we form a rigid body $\mathds{B}_R$ of $n$ nodes such that the length of each edge incident with a pair of nodes equals the corresponding pairwise range in $\mathbf{D}$. To this end, we use Classical Multi-Dimensional Sampling (CMDS) \cite{cmds-paper}. This is a widely used algorithm to map $n$ nodes into Cartesian space given the pairwise distances among them. We briefly discuss the CMDS problem and algorithm here.
%
\\ \noindent \textbf{Multi-Dimensional Sampling (CMDS) Problem: }
Given a complete $n\times{}n$ matrix $\mathbf{D^2}$ of squared distances $d^2_{ij}$'s between node $i$ and $j$, CMDS problem is to find the $n\times{}d$ coordinate Matrix $\mathbf{X}$ that gives the location $\mathbf{x}_{i}$ of each node $i$ in $d$-dimensional Euclidean Space.

In matrix notation, this amounts to solving for $\mathbf{B}=\mathbf{XX^T}$ where $\mathbf{X^T}$ is the transpose of matrix $\mathbf{X}$. As shown in \cite{cdms-paper}, $\mathbf{X}$ can be calculated as follows:
\begin{equation}
    \mathbf{D^2}=\mathbf{C\,1^T}+\mathbf{1\,C^T}-2\mathbf{XX^T}
    \label{eq-dsquare}
\end{equation}
Here, $\mathbf{C}$ is the $n\times{}1$ matrix with only the diagonal elements of $\mathbf{XX^T}$ and $\mathbf{1}$ is the $n\times{}1$ matrix of ones. By multiplying both sides of Equation \ref{eq-dsquare} by the centering matrix $\mathbf{J}=\mathbf{I}-\frac{1}{n}\mathbf{1\,1^T}$, we have
%
\begin{equation}
\begin{split}
    & -\frac{1}{2}\mathbf{JD^2J} =  -\frac{1}{2}\mathbf{J}( \mathbf{C\,1^T}+\mathbf{1\,C^T}-2\mathbf{XX^T} )\mathbf{J} 
    \\
    & = -\frac{1}{2}\mathbf{J\,C\,1^T\,J}-\frac{1}{2}\mathbf{J\,1\,C^T\,J}+\frac{1}{2}\mathbf{J}(2\mathbf{B})\mathbf{J} 
    \\
    & \mbox{ [centering $\mathbf{1}$ by $\mathbf{J}$ yields zero matrix i.e,  $\mathbf{1^T\,J}=\mathbf{J\,1}=\mathbf{0}$ ]}
    \\
    & = -\frac{1}{2}\mathbf{J\,C\, 0}-\frac{1}{2}\mathbf{0\,C^T\,J}+\mathbf{J\,B\,J}
    \\
    & = \mathbf{0}+\mathbf{0}+\mathbf{B} = \mathbf{B} 
    %\mbox{ [double-centering $\mathbf{B}$ by $\mathbf{J}$ gives $\mathbf{B}$ i.e. $\mathbf{J\,B\,J}=\mathbf{B}$}
     \\
    %& \mbox{ \hspace{1.5in} since $\mathbf{X}$ is column-centered, so is $\mathbf{B}$] }
    \\
    & \implies \mathbf{XX^T} = \mathbf{B}  = -\frac{1}{2}\mathbf{JD^2J} = \mathbf{Q}\,\Lambda\,\mathbf{Q^T} 
    %\mbox{ [Eigenvalue decomposition] }  
    \\
    & \implies \mathbf{X} = \mathbf{Q}\sqrt{\Lambda} 
\end{split}
\end{equation}
Therefore, CMDS algorithm involves the following 3 steps-
\\ \noindent 
I) Given square-distance matrix $\mathbf{D^2}$, compute Gram matrix $\mathbf{B}$ of $\mathbf{X}$ as $\mathbf{B}=-\frac{1}{2}\mathbf{JD^2J}$,
\\ \noindent 
II) Find the Eigenvalue decomposition of $\mathbf{B}=\mathbf{Q}\,\Lambda\,\mathbf{Q^T}$, 
\\ \noindent 
III) Finally, compute $\mathbf{X}=\mathbf{Q}\sqrt{\Lambda} $ for Eigenvector matrix $\mathbf{Q}$ and diagonal Eigenvalue matrix $\Lambda$.
\\
Due to the ``centering" assumption, each column of solution $\mathbf{X}$ sums to zero i.e, the origin of $\mathbf{X}$ coincides with the centroid of the $n$ locations. To derive the absolute location, we multiply $\mathbf{X}$ with the transformation matrix $\mathbf{M}$ to drive the absolute location. Section \ref{absolute-loc} describes it in detail.
Note that CMDS minimizes the loss function (also called \textit{strain}) $L( \mathbf{X} ) = ||\mathbf{XX^T} - \mathbf{B}||=||\mathbf{XX^T} - \frac{1}{2}\mathbf{JD^2J}||$. As such, the CMDS can end up in local minima. These local minima is more likely to occur when dimension is low (2 or 3 as in our case) \cite{cmds-book}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Rigid-body Formation Relative Localization}
We represent the network of nodes by a undirected graph $G_c$(V, $E_c$) where V represents the set of nodes and $E_c$ represents the set of edges or connectivity links between individual nodes. Connectivity links indicate reachability between two nodes and are determined by the nodes overhearing other nodes when the latter transmit. Note that $E_c$ is dynamic and depends on the relative location of the individual nodes. Let $G_m$ denote the measurement graph, given by $G_m$(V, $E_m$), where $E_m \subseteq E_c$. For each edge, $e_i \in E_m$, we estimate a \textit{measurement-tuple}, $M_{e_i}$ = $<R_{e_i}, t_{e_i}>$. $R_{e_i}$ is the range estimate or the inter-node distance obtained at time instant $t_{e_i}$. At any time instant $t$, we construct a spatial embedding of the nodes $V$ from the graph $G_m$. We call such an embedding, a rigid body $L_{rigid}^t = \texttt{rigid}( G_m )$, that provides relative localization of the individual nodes. Our objective is to minimize $|L^t - L_{rigid}^t|$, where $L^t$ denotes the `true' relative localization of the nodes in $V$ at time $t$.

We divide the time through which the system operates into slots. Each slot allows enough time to profile a single edge and update $L_{rigit}^t$. In essence, the problem boils down to a scheduling problem that intelligently selects and estimates $M_{e_i}$ at each time slot.
\smallskip

\noindent\textbf{Edge Uncertainty:} At the $T^{th}$ time slot, we define {\em staleness} of an edge $e_i$ as $s_i = (T - t_{e_i})$. Intuitively, higher the value of $s_i$, higher is the uncertainty associated with the measurements in $M_{e_i}$. For modeling such uncertainty we take a Bayesian approach. We maintain a table ($\texttt{TAB}_{edge}$) that, for any edge $e_i$, maps the time interval between two successive $M_{e_i}$s to the change in the estimated ranges. For instance, let $M_{e_i}^1$ and $M_{e_i}^2$ be two successive measurements obtained at time slots $t_1$ and $t_2$. We record the mapping $(t_2 - t_1) \rightarrow |R_{e_i}^2 - R_{e_i}^1|$ or, $\Delta t_i \rightarrow \Delta R_i$. At the $T^{th}$ time slot, we define edge uncertainty for edge $e_i$ as,
\begin{equation}
\label{eqn:edge_uncertainty}
	 U_{edge}^i = \texttt{Prob}( \Delta R > R_{threshold} | \Delta t = s_i)
\end{equation}
where $s_i$ is the current edge staleness and $R_{threshold}$ is the maximum $\Delta R$ the system can tolerate which is given as an input parameter to the system. Equation (\ref{eqn:edge_uncertainty}) can be easily computed from $\texttt{TAB}_{edge}$. When an edge E gets included in $E_c$, we create $\texttt{TAB}_{E}$ and maintain its history. When E is excluded from $E_c$ (i.e., E is no longer a valid connectivity link), we reset $\texttt{TAB}_{E}$.
\smallskip 

\noindent\textbf{Node Uncertainty:} We need {\em at least} three edges ($\in E_m$) incident on a node to make it a part of the rigid body, $L_{rigid}$. Consider a situation where out of several edges incident on a node $n_i$, three edges have low edge uncertainties ($U_{edge}$(s)). Although the remaining edges have high uncertainties, measuring those edges might not be best use of resources as the benefit that it will bring to the node $n_i$ in question might be minimal. We define node uncertainty as,
\begin{equation}
\begin{aligned}
	U_{node}^i &= \frac{u_1 + u_2 + u3}{3} \\
 u_1, u_2, u_3 &= min_3 \{ U_{edge}^{i1}, U_{edge}^{i2}, \cdots, U_{edge}^{iN} \} 	 
\end{aligned}
\end{equation}
where $i1, i2, \cdots, iN$ are the $N$ incident edges on node $n_i$. If $N \leq 2$, $u_3 = 1$ and/or $u_2 = 1$ respectively.

Initially, when adequate ranging information is not available to estimate the edge uncertainties ($U_{edge}$), we computer the node uncertainty ($U_{node}$) directly using IMU sensor data. A node's accelerometer information is used to track its total displacement, $D_i$. Under such circumstances, we define node uncertainty as,
\begin{equation}
\label{eqn:imu_uncertain}
 U_{node}^i = \frac{D_i}{R_{threshold}}
\end{equation}
 
\subsection{Algorithm Sketch}
In the following, we describe the different steps involved in the \system{'s} algorithm for relative localization.

\mypara{Bootstrap Phase:}
\begin{packedenumerate}
	\item \ul{\em Connectivity Graph:} Every node sequentially broadcasts a neighborhood discovery frame. This frame is overheard by the remaining nodes which helps every node determining its neighbors. Consequently, the graph $G_c$ is constructed using the neighborhood information.
	
	\item \ul{\em Ranging:} $U_{node}^i$ is calculated for each node $n_i$. Since enough historical information is not available, equation (\ref{eqn:imu_uncertain}) is used to estimate the same. The nodes are sorted according to their uncertainty values. Let the ordering be denoted by $[n_1, n_2, \cdots, n_{|V|-1}, n_{|V|}]$ s.t., $[U_{node}^{n_1} \leq U_{node}^{n_2} \cdots U_{node}^{n_{|V|-1}} \leq U_{node}^{n_{|V|}}]$. Next the following edges are ranged: $(n_1, n_{|V|})$, $(n_2,  n_{|V|-1})$ and so on, i.e., the node with the highest uncertainty is ranged with the one with the lowest and likewise.	
\end{packedenumerate}

\mypara{Steady State:}
For every time instant, T:
\begin{packedenumerate}
	
	\item \ul{\em Update:} Based on the latest measurement taken at $(T-1)$, new edges are created or removed from $E_c$. Accordingly, $G_c$ is updated. Depending on the measured edge at $(T-1)$, the corresponding table  $\texttt{TAB}_{edge}$ is updated. The value of $U_{edge}$ is and $U_{node}s$ are updated.
	
	\item \ul{\em Edge Selection:} We select the edge that induces maximum relative improvement on node uncertainty. (see Algorithm (1)) 
	
	\item \ul{\em EDM Update:} Only entries corresponding to the edges that are in $E_c$ are kept in the EDM. The rest of the entries are considered missing. The missing entries are predicted by a standard matrix completion algorithm based on {\em semi-definite rank relaxation} (SDR). Our edge selection mechanism is aware of the underlying rigid body and hence helps the SDR algorithm to predict missing entries with greater accuracy.
	
	\item \ul{\em Rigid-body Formation:} Once the EDM is complete, we run {\em multi dimensional scaling} (MDS) on it to estimate $L_{rigid}^T$. Discussion about IMU will also come here how we apply MDS.
\end{packedenumerate}

\begin{algorithm}
	\caption{Edge Selection}
	\begin{algorithmic}
		\STATE try out every edge and see which edge creates the maximum relative benefit for the node-pair. select that edge. 
	\end{algorithmic}
\end{algorithm}

==> oldabslocalization.tex <==
The relative locations was calculated with respect to an arbitrary local axis. We have to perform translational, rotation and flip or a combination of them to align this local axis with a global axis. Ideally, we'd require locations of at least 3 nodes in the rigid graph with respect to global axis to do the transformation. However, that is too demanding on the dynamic indoor environment. Instead, we require that only one node will be static (can be put at the main-doors or other known landmark). Based on that, we apply translation, rotation and flip as using the heading data from IMU as follows.

\begin{figure}[!htb]
	\centering
	\subfloat[Line-heading]
	{
		\includegraphics[width=0.4\linewidth]{figs/section-3-plots/abs-loc-rot}
		\label{fig:abs-loc-rot}
	}
	\subfloat[Flip correction]
	{
		\includegraphics[width=0.6\linewidth]{figs/section-3-plots/vertex-ordering}
		\label{fig:abs-loc-flip}
	}
	\caption{Absolute localization}
	\label{fig:abs-loc}
\end{figure}
%
\noindent \textit{\underline{Fixing Translation}}: We make the fixed node as the origin of the global axis by subtracting its coordinate from all relative locations.
%
\\ \noindent \textit{\underline{Fixing Rotation}}: After fixing translation, we rotate the relative axes to align with the global ones by applying the transformation: $x^{'} = [ x\cos\theta-y\sin\theta]$ and $y^{'} = [ x\sin\theta+y\cos\theta]$ after determining the rotation angle $\theta$ as follows. We assume that the global x-axis is aligned with the earth's north-south magnetic axis in the horizontal plane. Therefore, we set $\theta$ to be the angle between the relative x-axis and the north-south axis. For this we assume that when the nodes are in motion, their heading\footnote{Here, heading is the angle with the earth's magnetic north-south axis on the horizontal plane, as read from the IMU. When a node is fixed, its pose can be in any direction, however when it is in motion, the pose is generally in the direction of the motion}, as read from the IMU,  aligns with their direction of the motion. We can construct a polar coordinate $(r_i, \theta_i)$ for each node $i$, where $r_i$ is the distance (already computed in the previous steps) from the fixed node and $\theta_i$ is their heading. We then compute the ``banking" angle of any edge  in the rigid graph with earth's north-south axis from the geometry of the polar coordinate. As shown in Figure \ref{fig:abs-loc-rot}, the banking angle of edge (2,3) is computed using distances $r_{12}, r_{13}$ and headings $\theta_2$, $\theta_3$.  We then find the angle $\theta^{'}_{23}$ that this edge makes with the +ve x-axis in the relative coordinate system and compute the rotation angle as $(\theta_{23} - \theta^{'}_{23})$. We  calculate the banking angle for each edge with whose incident nodes are mobile (our assumption of aligned heading \& direction of motion holds) and compute the required rotation angle from each of the banking angles. We then take average of all these rotation angles as the final rotation to be applied on the relative coordinate system.
%
\\ \noindent \textit{\underline{Fixing Flip}}: For any graph, we can derive a vertex-ordering based on the  slope of the line segment connecting the node and the centroid (average) of their locations. As shown in Figure \ref{fig:abs-loc-flip}, the two rigid graphs are flip or mirror image of each other. Their vertex-ordering w.r.t. the centroid in counter-clockwise direction are different (1-2-3-4-5 vs 1-5-4-3-2). We compute the vertex ordering both in the  polar coordinate (which is the correct ordering based on the heading information) and the relative coordinate. If the two ordering does not agree, the rigid graph has been flipped during construction. We correct the flip by inverting the polarities of the x-coordinate. This check and correction is done before applying the rotation.
%
\begin{figure}[!htb]
	\centering
		\includegraphics[width=0.75\linewidth]{figs/section-3-plots/floorplan}
	\caption{Embedding on a floormap}
	\label{fig:abs-floormap}
\end{figure}
%
\\ \textit{\underline{Embedding on the floormap}}: Additionally, it is desirable to show the location on a given floormap. In this case, no fixed node is required. An arbitrary node is treated as a fixed origin of the relative coordinate and applied translation, rotation, flip correction as before. Additionally, we store the history of locations called tracks, of individual nodes over time.  Two such tracks are shown in Figure \ref{fig:abs-floormap}. We treat the set of tracks as a rigid graph and try to embed the graph on the floormap with no crossing with the walls by considering  all possible translation of the graph within the bounding box of the floormap. As such, the rooms, hallways etc. of the indoor area put additional constraints on the localization via this embedding. There can be multiple candidates for the embedding if the tracks are short or the indoor space lacks distinct paths itself. Otherwise, the floormap removes the requirement of a fixed node.

==> optical-tracking.tex <==
%optical tracking
{\color{brown}
\subsection{Motivation for RF-based localization in dynamic infrastructure-free environments}
%
%what is dynamic environment
%
%infrastructure-free
	%not device-free passive localization, using radar etc
	
%dynamic environment- example -localization what are the usecases- public safety, VR, live-entertainment>>geographic limitation, on the fly---real drill instead of simulation
%why localization is important 
	%in dynamic environment
	%in infrastructure-free cases
	% use-cases: forward references from paper's applications
%already in use-
	%no fingerprinting, agains visual SLAM
	%1) IMU
	%2) Visual Odometry
	%3) VIO
%why the system would break?
	%in the above cases:10-20% will work
	%will fail the rest of the time
%now motivate RF-based techniques
%results: IMU- dead-reckoning, VIO failures

%latency: missed opportunity: real-time/interactive
	%missing 90% opportunity in applications
	%existing system 6-dof:does not support translation 

%HOW CAN RF MAKE THE SYSTEM BETTER?
	%SOLELY RF
	%ENHANCEMENT BY RF
%
%
%
Indoor localization is a well-studied problem \cite{indoor-loc-survey}. Due to poor or lack of reception of GPS, the solution for indoor localization often involves a host of technologies such as optical \cite{optical-loc-survey}, visual \cite{viz-loc-survey}, inertial \cite{intertial-loc-survey}, RF \cite{loc-survey} etc. We can categorize these solutions as ``active" and ``passive" localization. In active localization, the objects are identifiable \cite{passive-loc-ov} whereas in passive case, they are not \cite{loc-survey} (here, only the count of the tracked objects matter). This work pertains to only active localization, as such the identity of each localized object is essential. In particular, each tracked object or person carries a device that enables both the identification and localization of them. We further categorize the active localization in two groups- such as localization with and without infrastructure. In the solution with infrastructure \cite{loc-survey}, some designated devices are put at pre-computed location for optimal operation. These devices with fixed locations are called ``anchors". Depending on the technology used, anchors periodically transmit RF \cite{loc-survey} or infrared \cite{lidar-survey} beacons, which in turn enables the localization or tracking via a variety of methods, such as Time Difference of Arrival (TDOA)\cite{toda-ov}, Time of Flight (TOF) \cite{tf-ov} etc. in conjunction with multi-lateration \cite{multi-lat-ov}, fingerprint-matching \cite{fingerprinting-loc-survey} etc. In these applications, the deployment involves careful placement and calibration of the anchors \cite{vr-devs}. Dysfunction of a single anchor disable the localization system in entirety. Anchor-based real-time indoor localization service provided by companies such as \cite{loc-solution-survey} has been deployed in factories, warehouses etc. for many years.
%
Another broad area within active localization is based fingerprinting-based localization,  wherein- the area of interest is scanned beforehand using a variety of methods \cite{} and then the objects are localized by matching the fingerprints. However, any change in the environment necessitates re-collection of the fingerprints. 
%
Our work concerns indoor localization in a ``dynamic" environment, which is unknown, unmapped and unexplored and has a lot of moving parts to the extent that- i) the anchors cannot be deployed in pre-planned way ii) the environments cannot be fingerprinted beforehand and/or the fingerprints cannot be used reliably due to constant change in the environments. Assumption of such dynamic environments often is necessary for example in the case of tracking first responders such as firefighters \cite{tackio}, SWAT team \cite{swat-app} etc; sometimes the assumption is desirable for example, in case of Augmented and Virtual (AR/VR) reality applications, which currently requires meticulous placement and calibration of the controller plus the beacons \cite{vr-dev-survey}. In summary, dynamic indoor environment requires infrastructure-free solution that does not depend on fingerprinting. Our works pertains to active localization in GPS-denied dynamic indoor environments without fingerprinting and anchor-placement.
%
\begin{table}
\begin{center}
\begin{tabular}{|p{1.5cm}|p{2cm}|p{4cm}|}
%
\hline 
%
\textbf{Method} & \textbf{Pros} & \textbf{Cons} \\ \hline
Inertial Tracking (IT) & No anchor-deployment, inexpensive hardware & Run-away positional drift w/o periodic fix  \\ \hline
%
Optical Tracking (OT)  & Most precise (millimeter-level accuracy) & Requires LOS \& anchor-deployment, expensive hardware \\ \hline
%
Visual Odometry (VO) \cite{}, Visual Intertial Odometry (VIO) & accurate under favorable condition, no anchor-deployment & Suffers from runaway optical drift  w/o periodic sync, less accurate in low-light, poorly-textured environments , computationally extensive, requires expensive hardware  \\ \hline
%
\end{tabular}
\caption{Comparison of non-RF solutions for infrastructure-free indoor localization for dynamic indoor environments}
\end{center}
\label{tab:dyn-loc-sol}
\end{table}
\\
First, we turn to the candidate solutions that are not RF-based. Table \ref{tab:dyn-loc-sol} summarizes such solutions and their pros and cons in the context of dynamic environments. IT has been successfully used in automobile and robot navigation \cite{auto-nav} because of the deterministic displacement from the rotation-count of the wheels. However, pedestrian dead-reckoning \cite{ped-dr-survey} suffers from positional drifts without periodic fix. Facilitating periodic fix for each object at any arbitrary location is equivalent to dense infrastructure-deployment and is infeasible in our dynamic environment. The line-of-sight  requirement rules out the OT approach for our scenario since most indoor space has walls and obstacles. Finally, the VO/VIO approach requires camera plus IMU and can render sub-centimeter-level accuracy \cite{vio-dev-survey} under favorable condition. However, it suffers from a range of limitations such as:
\begin{enumerate}
%
 \item \textbf{Technological Limitation: }regardless of the instruments used, VIO system performs poorly (even fails completely) in poorly illuminated and/or poorly textured environments\cite{opto-survey}, in presence of motion-blur \cite{opto-blur} and/or multiple moving objects in the video-frames \cite{opto-obj} etc.
  \item \textbf{Sensor/Instrumental Limitations: }Sometimes to operate in challenging environments such as poorly illuminated and textured etc., VIO requires expensive camera/sensors \cite{vio-dev-survey} and high computation power. Inexpensive cameras \cite{vio-dev-survey} and low compute power typically renders poor accuracy \cite{vio-ins-acc}.
  \item \textbf{Algorithmic Limitations: }Finally, the algorithms for VIO also suffer from multitude of limitations. For example the SLAM-based algorithms \cite{vslam-ov} suffers from initialization error \cite{vlam-ov}, drift error \cite{vslam-st}, loop-closure error \cite{vslam-lce}, ``pure rotation" error \cite{vslam-rot-e}, scale ambiguity \cite{vslam-de} and so on. Other class of optical flow-based algorithms suffer from limitations related projection errors (3D-to-2D or 3D-to-3D) \cite{of-proj}, parameterization error \cite{of-overview}, vector-clustering error \cite{of-cluster-e} and so on. Finally quality of visual-feature selection, de-noising and filtering of the sensor data etc. also introduces additional errors \cite{of-feature-e}. All these types of errors accumulate over type to a point where the system breaks. Therefore, these kind of systems often incorporate periodic resetting mechanism and cross-validation \cite{of-augmentation} which is often infeasible in our dynamic unknown environments. 
  %
\end{enumerate}
%
Due to such limitations of VIO, we use RF both as a stand-alone and augmenting technology for localization in dynamic indoor environments.
\\
%
\begin{figure}[!htb]
	\centering
	\subfloat[]
	{
		\includegraphics[width=0.45\linewidth]{figs/rel-lit-1}
		\label{fig:infra-spectrum}
	}
	\subfloat[]
	{
		\includegraphics[width=0.45\linewidth]{figs/rel-lit-2}
		\label{robust-spectrum}
	}
	\caption{Accuracy of difference approaches in spectrum of (a) deployment overhead and (b) robustness. 
	}
	%\vspace{-0.8 cm}
\end{figure}
%
We can arrange all the works on localization on two broad categories 1) deployment overhead: precise infrastructure (anchors) placement on one end and totally infrastructure-free on the other end of the spectrum (See Figure \ref{fig:infra-spectrum} and 2) robustness: totally known/fingerprinted environment on one end and fully unknown environment on the other end of this spectrum (See Figure \ref{fig:robust-spectrum}. As evident from these figures, current literature is devoid of works in the dynamic unknown environments (shaded region of the two spectrum), let alone high-accuracy works for that region. Our work contribute to this un-addressed region of utility which encompasses a lot of applications in public safety, entertainment etc. as outlined in applications in Section \ref{sec:app}. With this clarity, we introduce our work for dynamic unknown environments. 
\\
}


==> related.tex <==
Localization system has been discussed in \cite{md-track-19}, \cite{monoloco-18}, \cite{chronos-16}, \cite{spotfi-15}, \cite{tonetrack-15}, \cite{ubicarse-14}, \cite{phaser-14}, \cite{tagogram-14}, \cite{lte-eye-14}, \cite{array-track-13}, \cite{pinpoint-13}, \cite{pin-it-13}, \cite{zee-12}, \cite{pin-loc-12}, \cite{ez-10}
